Dense Incremental Metric-Semantic Mapping for Multi-Agent Systems via Sparse Gaussian Process Regression

We develop an online probabilistic metric-semantic mapping approach for mobile robot teams relying on streaming RGB-D observations. The generated maps contain full continuous distributional information about the geometric surfaces and semantic labels (e.g., chair, table, wall). Our approach is based on online Gaussian Process (GP) training and inference, and avoids the complexity of GP classification by regressing a truncated signed distance function (TSDF) of the regions occupied by different semantic classes. Online regression is enabled through a sparse pseudo-point approximation of the GP posterior. To scale to large environments, we further consider spatial domain partitioning via an octree data structure with overlapping leaves. An extension to the multi-robot setting is developed by having each robot execute its own online measurement update and then combine its posterior parameters via local weighted geometric averaging with those of its neighbors. This yields a distributed information processing architecture in which the GP map estimates of all robots converge to a common map of the environment while relying only on local one-hop communication. Our experiments demonstrate the effectiveness of the probabilistic metric-semantic mapping technique in 2-D and 3-D environments in both single and multi-robot settings.

==> tex/IncGPreg.tex <==
%!TEX root = ../main.tex

\section{Incremental Gaussian Process Regression}
\label{sec:incGPreg}
We propose an efficient approach for \emph{incremental} GP regression which performs online training using streaming data. We assume that the kernel parameters are optimized offline and focus on online computation of the terms in~\eqref{eq:pseudopoint_gp_posterior}, needed for prediction. \medskip

%\subsection
{\noindent \bf Repeated Input Data Compression}
We first exploit the fact that if the data $\calD$ contains repeated observations from the same location, then the training complexity of a GP can be reduced from cubic in the number of observations $|\calD|$ to cubic in the number of distinct observed points. We formalize the mentioned fact in the following proposition, establishing that the GP posterior remains unchanged if we compress the training data obtained from the same locations.

\begin{proposition}
\label{prop:gp_compression}
Consider $f(\bfx) \sim \mathcal{GP}(\mu_0(\bfx), k_0(\bfx,\bfx')$. Let:
%
\begin{equation}
\label{eq:original_data}
\begin{aligned}
%
\calX&=\{\bfx_1\;\;, \ldots,\bfx_1\;\;\;\;, \bfx_2\;\;,\ldots,\bfx_2\;\;\;\;,\ldots,\bfx_n\;\;,\ldots,\bfx_n\;\;\;\;\}\\
\bfy&=\brl{y_{1, 1}, \ldots, y_{1, m_1}, y_{2, 1}, \ldots, y_{2, m_2}, \ldots, y_{n, 1}, \ldots, y_{n, m_n}}^\top
%
\end{aligned}
\end{equation}
%
be data generated from the model $y_{i, j} = f(\bfx_i) + \eta_{i,j}$ with $\eta_{i,j} \sim \mathcal{N}(0, \sigma^2)$ for $i=1,\ldots, n$ and $j = 1,\ldots, m_i$. Let:
%
\begin{equation}
\label{eq:compressed_data}
\begin{aligned}
%
\calP = \{\bfx_1, \ldots, \bfx_n\}, \;  
\bfzeta = \brl{ \frac{1}{m_1} \sum_{j=1}^{m_1} y_{1, j}, \ldots, \frac{1}{m_n} \sum_{j=1}^{m_n} y_{n, j} }^\top
%
\end{aligned}
\end{equation}
%
be a compressed version of the data generated from $f(\bfx_i)$ with noise $\hat{\eta}_{i} \sim \mathcal{N}(0, \frac{\sigma^2}{m_i})$. Then, $f(\bfx) | \calX,\bfy$ and $f(\bfx) | \calP, \bfzeta$ have the same Gaussian Process distribution $\mathcal{GP}(\mu(\bfx),k(\bfx,\bfx'))$ with:
%
\begin{equation}
\label{eq:compressed_gp_posterior}
\begin{aligned}
\mu(\bfx) &= \mu_0(\bfx) + k_0(\bfx, \calP) Z(\bfzeta - \mu_0(\calP)),\\
k(\bfx,\bfx') &=  k_0(\bfx, \bfx') - k_0(\bfx, \calP) Z k_0(\calP, \bfx'),
\end{aligned}
\end{equation}
%
where $Z^{-1} := k_0(\calP, \calP) + \sigma^2\diag(\bfm)^{-1}$ and $\bfm$ is a vector with elements $m_i$.
\end{proposition}

\begin{proof}
The distribution of $f(\bfx) | \calX,\bfy$ is provided in~\eqref{eq:gp_posterior}. Using the data $\calP$, $\bfzeta$, instead of $\calX$, $\bfy$, to compute the posterior GP distribution of $f(\bfx)$, according to~\eqref{eq:gp_posterior}, leads to the expression in~\eqref{eq:compressed_gp_posterior}. We need to show that~\eqref{eq:gp_posterior} and~\eqref{eq:compressed_gp_posterior} are equal given the relationship between $\calX$, $\bfy$ and $\calP$, $\bfzeta$ in~\eqref{eq:original_data} and~\eqref{eq:compressed_data}. Let $E$ be a binary matrix defined such that $k_0(\calX,\bfx) = E k_0(\calP,\bfx)$. Note that $k_0(\calX,\calX) = E k_0(\calP,\calP)E^\top$, $k_0(\bfx,\calX) = k_0(\bfx,\calP)E^\top$, $E^\top E = \diag(\bfm)$, and $\bfzeta = (E^\top E)^{-1} E^\top \bfy$. Using these expressions in~\eqref{eq:gp_posterior} leads to:
%
\begin{align}\label{eq:E_gp_posterior}
\mu(\bfx) &= \mu_0(\bfx) +\notag\\ 
&k_0(\bfx, \calP)E^\top (Ek_0(\calP, \calP)E^\top+ \sigma^2 I)^{-1}(\bfy - E\mu_0(\calP)),\notag\\
k(\bfx,\bfx') &=  k_0(\bfx, \bfx') - \\
&k_0(\bfx, \calP)E^\top (Ek_0(\calP, \calP)E^\top + \sigma^2 I)^{-1} Ek_0(\calP, \bfx').\notag
\end{align}
%
An application of the matrix inversion lemma followed by algebraic manipulation shows that $E^\top (Ek_0(\calP, \calP)E^\top + \sigma^2 I)^{-1} = \prl{k_0(\calP, \calP) + \sigma^2 (E^\top E)^{-1}}^{-1} (E^\top E)^{-1}E^\top = Z (E^\top E)^{-1}E^\top$. Replacing this and $\bfzeta = (E^\top E)^{-1} E^\top \bfy$ in~\eqref{eq:E_gp_posterior} shows that the GP distributions of $f(\bfx) | \calX,\bfy$ and $f(\bfx) | \calP, \bfzeta$ are equal.
\end{proof}

Prop.~\ref{prop:gp_compression} allows us to summarize a training set $\calX$, $\bfy$ by keeping the distinct pseudo points $\calP$, the average observation value $\zeta(\bfp)$, and the number of times $m(\bfp)$ that each points $\bfp \in \calP$ has been observed. Given these statistics, the mean function $\mu(\bfx)$ and covariance function $k(\bfx,\bfx')$ of the posterior GP can be obtained according to~\eqref{eq:compressed_gp_posterior} with $\bfzeta := \zeta(\calP)$ and $\bfm := m(\calP)$. This leads to significant computational savings when the pseudo points $\calX$ contain repetitions. We will exploit this compression technique for efficient incremental learning when the same locations are observed multiple times online. \medskip



%\subsection
{\bf \noindent Incremental GP Updates}
%
Suppose now that, instead of a single training set, the data are provided sequentially, i.e., an additional dataset $\tilde{\calD}_t$ of pseudo points $\tilde{\calX}_t$ with labels $\tilde{\bfy}_t$ is provided at each time step $t$ so that the cumulative data up to time $t$ are $\calD_t := \cup_{\tau = 1}^t \tilde{\calD}_\tau$. Based on Prop.~\ref{prop:gp_compression}, we can define an incrementally growing set of pseudo points $\calP_t$ with associated number of observations $m_t(\bfp)$ and average observation $\zeta_t(\bfp)$ for $\bfp \in \calP_t$ and observation precision $Z_t$. We show how to update these statistics when a new dataset $\tilde{\calX}_{t+1}$, $\tilde{\bfy}_{t+1}$ arrives at time $t+1$. Let $\tilde{\calP}_{t+1}$ be the set of unique points in $\tilde{\calX}_{t+1}$ with number of observations $\tilde{m}_{t+1}(\bfp)$ and average observation $\tilde{\zeta}_{t+1}(\bfp)$ for $\bfp \in \tilde{\calP}_{t+1}$. The update of $\calP_t$, $m_t(\bfp)$ and $\zeta_t(\bfp)$ is straightforward:
\begin{equation}
\label{eq:update}
\begin{aligned}
\calP_{t+1} &= \calP_t \cup \tilde{\calP}_{t+1}\\
m_{t+1}(\bfp) &= \begin{cases}
      m_t(\bfp) + \tilde{m}_{t+1}(\bfp), & \text{if } \bfp \in \calP_t,\\
      \tilde{m}_{t+1}(\bfp), & \text{else},
      \end{cases}\\
\zeta_{t+1}(\bfp) &= \begin{cases}
      \frac{m_t(\bfp)\zeta_t(\bfp) + \tilde{m}_{t+1}(\bfp)\tilde{\zeta}_{t+1}(\bfp)}{m_{t+1}(\bfp)}, & \text{if } \bfp \in \calP_t,\\
      \tilde{\zeta}_{t+1}(\bfp), & \text{else}.
      \end{cases}
\end{aligned}
\end{equation}
%\frac{\prl{m_t(\bfp)\zeta_t(\bfp) + \tilde{m}_{t+1}(\bfp)\tilde{\zeta}_{t+1}(\bfp)}}{m_{t+1}(\bfp)}
To update the observation precision $Z_t$, first consider the existing pseudo points $\calP_t$. Let $l$ be the index of $\bfp \in \calP_t$ in $Z_t$. Define $\epsilon_l := \frac{\sigma^2}{m_{t+1}(\bfp)} - \frac{\sigma^2}{m_{t}(\bfp)}$, $B_0 := Z_t$, and for $l = 1,\ldots,|\calP_t|$:
\begin{equation}
\label{eq:precisionUpdate1}
B_{l+1} = \prl{B_l^{-1} +  \epsilon_l \bfe_l \bfe_l^\top}^{-1} = B_l - \frac{B_l \bfe_l \bfe_l^\top B_l}{\frac{1}{\epsilon_l} + \bfe_l^\top B_l \bfe_l}.
\end{equation}
With some abuse of notation, let $B := B_{|\calP_t|}$ be the observation precision after all $\bfp \in \calP_t$ have been updated. Finally, we update $B$ by introducing the pseudo points $\tilde{\calP}_{t+1}\setminus \calP_t$ that have been observed for the first time:
\begin{equation}
\label{eq:precisionUpdate2}
Z_{t+1} = \begin{bmatrix} B^{-1} & C\\ C^\top & D \end{bmatrix}^{-1} = \begin{bmatrix} B + BCSC^\top B & -BCS\\ -S C^\top B & S \end{bmatrix},
\end{equation}
where $C := k_0(\calP_t,\tilde{\calP}_{t+1}\setminus \calP_t)$, $D := k_0(\tilde{\calP}_{t+1}\setminus \calP_t,\tilde{\calP}_{t+1}\setminus \calP_t) + \sigma^2 \diag(\tilde{m}_{t+1}(\tilde{\calP}_{t+1}\setminus \calP_t))^{-1}$, and $S := (D  - C^\top B C)^{-1}$. By recursively tracking these matrix inverses, the posterior update can be executed efficiently every time a new observation arrives with complexity that is cubic in the number of new distinct points. This is a significant reduction; however, it is not enough to facilitate scaling to large spaces. For this purpose, we employ specific structural decompositions of the space using Octree. This aspect, as well as how the training set is constructed from the robotic observations discussed in Sec. \ref{sec:problem_formulation} are the focus of the following section.































==> tex/NikolaysAddon.tex <==
%!TEX root = ../main.tex

\section{Sparse Gaussian Process Regression}

A \emph{Gaussian Process} (GP) is a set of random variables such that the joint distribution of any finite subset of them is Gaussian. A GP-distributed function $f(\bfx) \sim \mathcal{GP}(\mu_0(\bfx), k_0(\bfx, \bfx'))$ is defined by a mean function $\mu_0(\bfx)$ and a covariance (kernel) function $k_0(\bfx, \bfx')$. The mean and covariance are such that for any finite set $\calX = \crl{\bfx_1,\ldots,\bfx_M}$, the random vector $f(\calX) := \brl{f(\bfx_1),\ldots,f(\bfx_M)}^\top \in \mathbb{R}^{M}$ has mean with $j$-th element $\mu_0(\bfx_j)$ and covariance matrix with $(j,l)$-th element $k_0(\bfx_j, \bfx_l)$ for $j,l = 1,\ldots,M$. Given a training set $\calD=\{(\bfx_j, y_j)\}_{j=1}^M$, generated according to $y_j=f(\bfx_j)+\epsilon_j$ with independent Gaussian noise $\epsilon_j \sim \calN(0, \sigma^2)$, the posterior distribution of the random function $f(\bfx)$ can be obtained from the joint distribution of the value $f(\bfx)$ at an arbitrary location $\bfx$ and the random vector $\bfy := \brl{y_1,\ldots,y_M}^\top$ of measurements. In detail, the joint distribution is:
\begin{equation}
\begin{aligned}
\begin{bmatrix} f(\bfx) \\ \bfy \end{bmatrix} \sim \mathcal{N}\prl{ \begin{bmatrix} \mu_0(\bfx) \\ \mu_0(\calX) \end{bmatrix}, \begin{bmatrix} k_0(\bfx,\bfx) & k_0(\bfx, \calX)\\
k_0(\calX,\bfx) & k_0(\calX,\calX) + \sigma^2 I\end{bmatrix}},
\end{aligned}
\end{equation}
while the corresponding conditional distribution $f(\bfx)|\calD \sim \mathcal{GP}(\mu(\bfx), k(\bfx, \bfx'))$ has mean and covariance functions:
%
\begin{equation}
\label{eq:gp_posterior}
\begin{aligned}
\mu(\bfx) &:= \mu_0(\bfx) + k_0(\bfx, \calX) (k_0(\calX, \calX)+ \sigma^2 I)^{-1}(\bfy - \mu_0(\calX)),\\
k(\bfx,\bfx') &:=  k_0(\bfx, \bfx') - k_0(\bfx, \calX) (k_0(\calX, \calX) + \sigma^2 I)^{-1} k_0(\calX, \bfx').
\end{aligned}
\end{equation}
%
Computing the GP posterior has cubic complexity in the number of observations $M$ due to the matrix inversion in~\eqref{eq:gp_posterior}.


Snelson and Ghahramani~\cite{snelson2006sparse} introduced a sparse approximation to the GP posterior in~\eqref{eq:gp_posterior} using a set of \emph{pseudo inputs} $\calP$. The key idea is to first determine the distribution $\calN\prl{\bfmu,\Sigma}$ of $\bff := f(\calP)$ conditioned on $\calX$, $\bfy$ according to~\eqref{eq:gp_posterior}:
\begin{equation}
\label{eq:pseudopoint_distribution}
\begin{aligned}
\bfmu &:= \mu_0(\calP) + k_0(\calP, \calX) (k_0(\calX, \calX)+ \sigma^2 I)^{-1}(\bfy - \mu_0(\calX))\\
 &\phantom{:}= \mu_0(\calP) + k_0(\calP,\calP)\prl{k_0(\calP,\calP) + \Gamma}^{-1}k_0(\calP,\calX) \prl{\Lambda + \sigma^2 I}^{-1}(\bfy - \mu_0(\calX))\\
\Sigma &:=  k_0(\calP,\calP) - k_0(\calP,\calX)\prl{ k_0(\calX,\calX) + \sigma^2 I }^{-1} k_0(\calX,\calP),\\
 &\phantom{:}= k_0(\calP,\calP)\prl{k_0(\calP,\calP) + \Gamma}^{-1}k_0(\calP,\calP)
\end{aligned}
\end{equation}
where $\Gamma := k_0(\calP,\calX)\prl{\Lambda + \sigma^2 I}^{-1}k_0(\calX,\calP)$ and $\Lambda := k_0(\calX,\calX) - k_0(\calX,\calP) k_0(\calP,\calP)^{-1} k_0(\calP,\calX)$. 
%where $\Lambda(X_n)$ is a diagonal matrix with entries $\lambda(\bfx_j) := k_0(\bfx_j,\bfx_j) - k_0(\bfx_j,P_n)k_0(P_n,P_n)^{-1} k_0(P_n,\bfx_j)$ on the diagonal.
Then, the posterior of $f(\bfx)$ conditioned on $\calX, \bfy$ is:
\begin{equation}
p( f(\bfx) | \calX, \bfy) = \int p(f(\bfx) | \bff) p(\bff | \calX, \bfy) d\bff
\end{equation}
which is a GP with mean and covariance functions:
\begin{equation}
\label{eq:pseudopoint_gp_posterior}
\begin{aligned}
\mu(\bfx) &= \mu_0(\bfx) + k_0(\bfx, \calP)k_0(\calP,\calP)^{-1}\prl{\bfmu - \mu_0(\calP)}\\
&=\mu_0(\bfx) + k_0(\bfx, \calP)\prl{k_0(\calP,\calP) + \Gamma}^{-1}k_0(\calP,\calX)\prl{\Lambda + \sigma^2 I}^{-1}(\bfy - \mu_0(\calX))\\
k(\bfx,\bfx') &= k_0(\bfx,\calP) k_0(\calP,\calP)^{-1}\Sigma k_0(\calP,\calP)^{-1} k_0(\calP,\bfx') + k_0(\bfx,\bfx') - k_0(\bfx,\calP)k_0(\calP,\calP)^{-1}k_0(\calP,\bfx')\\
&=k_0(\bfx,\calP) \prl{k_0(\calP,\calP) + \Gamma}^{-1} k_0(\calP,\bfx') + k_0(\bfx,\bfx') - k_0(\bfx,\calP)k_0(\calP,\calP)^{-1}k_0(\calP,\bfx').
\end{aligned}
\end{equation}
If we assume that conditioned on $\calP$, the measurements $y_j$ are generated independently, i.e., $\Lambda$ is approximated by a diagonal matrix with elements $\lambda(\bfx_j) := k_0(\bfx_j,\bfx_j) - k_0(\bfx_j,\calP)k_0(\calP,\calP)^{-1}k_0(\calP,\bfx_j)$, then the complexity of computing $\bfmu$, $\Sigma$ in~\eqref{eq:pseudopoint_distribution} (training) and $\mu(\bfx)$, $k(\bfx,\bfx')$ in~\eqref{eq:pseudopoint_gp_posterior} (testing) are $O(|\calP|^2 |\calX| + |\calP|^3)$ and $O(|\calP|^2)$, respectively, instead of $O(|\calX|^3)$ and $O(|\calX|^2)$ without pseudo inputs in~\eqref{eq:gp_posterior}. The use of pseudo inputs leads to significant computational savings when $|\calP| \ll |\calX|$.



\section{Incremental GP Regression}
We propose an efficient approach for \emph{incremental} GP regression which performs online training using streaming data. We assume that the kernel parameters are optimized offline and focus on online computation of the terms in~\eqref{eq:pseudopoint_gp_posterior}, needed for prediction. 

\subsection{Repeated Input Data Compression}
Our idea is based on a key observation that if the data $\calD$ contains repeated observations from the same location, then the training complexity of a GP can be reduced from cubic in the number of observations $|\calD|$ to cubic in the number of distinct observed points. We formalize this in the following proposition, establishing that the GP posterior remains unchanged if we compress the training data obtained from the same locations.

\begin{proposition}
\label{prop:gp_compression}
Consider $f(\bfx) \sim \mathcal{GP}(\mu_0(\bfx), k_0(\bfx,\bfx')$. Let:
%
\begin{equation}
\label{eq:original_data}
\begin{aligned}
%
\calX&=\{\bfx_1\;\;, \ldots,\bfx_1\;\;\;\;, \bfx_2\;\;,\ldots,\bfx_2\;\;\;\;,\ldots,\bfx_n\;\;,\ldots,\bfx_n\;\;\;\;\}\\
\bfy&=\brl{y_{1, 1}, \ldots, y_{1, m_1}, y_{2, 1}, \ldots, y_{2, m_2}, \ldots, y_{n, 1}, \ldots, y_{n, m_n}}^\top
%
\end{aligned}
\end{equation}
%
be data generated from the model $y_{i, j} = f(\bfx_i) + \eta_{i,j}$ with $\eta_{i,j} \sim \mathcal{N}(0, \sigma^2)$ for $i=1,\ldots, n$ and $j = 1,\ldots, m_i$. Let:
%
\begin{equation}
\label{eq:compressed_data}
\begin{aligned}
%
\calP = \{\bfx_1, \ldots, \bfx_n\}, \;  
\bfzeta = \brl{ \frac{1}{m_1} \sum_{j=1}^{m_1} y_{1, j}, \ldots, \frac{1}{m_n} \sum_{j=1}^{m_n} y_{n, j} }^\top
%
\end{aligned}
\end{equation}
%
be a compressed version of the data generated from $f(\bfx_i)$ with noise $\hat{\eta}_{i} \sim \mathcal{N}(0, \frac{\sigma^2}{m_i})$. Then, $f(\bfx) | \calX,\bfy$ and $f(\bfx) | \calP, \bfzeta$ have the same Gaussian Process distribution $\mathcal{GP}(\mu(\bfx),k(\bfx,\bfx'))$ with:
%
\begin{equation}
\label{eq:compressed_gp_posterior}
\begin{aligned}
\mu(\bfx) &= \mu_0(\bfx) + k_0(\bfx, \calP) Z(\bfzeta - \mu_0(\calP)),\\
k(\bfx,\bfx') &=  k_0(\bfx, \bfx') - k_0(\bfx, \calP) Z k_0(\calP, \bfx'),
\end{aligned}
\end{equation}
%
where $Z^{-1} := k_0(\calP, \calP) + \sigma^2\diag(\bfm)^{-1}$ and $\bfm$ is a vector with elements $m_i$.
\end{proposition}

\begin{proof}
The distribution of $f(\bfx) | \calX,\bfy$ is provided in~\eqref{eq:gp_posterior}. Using the data $\calP$, $\bfzeta$, instead of $\calX$, $\bfy$, to compute the posterior GP distribution of $f(\bfx)$, according to~\eqref{eq:gp_posterior}, leads to the expression in~\eqref{eq:compressed_gp_posterior}. We need to show that~\eqref{eq:gp_posterior} and~\eqref{eq:compressed_gp_posterior} are equal given the relationship between $\calX$, $\bfy$ and $\calP$, $\bfzeta$ in~\eqref{eq:original_data} and~\eqref{eq:compressed_data}. Let $E$ be a binary matrix defined such that $k_0(\calX,\bfx) = E k_0(\calP,\bfx)$. Note that $k_0(\calX,\calX) = E k_0(\calP,\calP)E^\top$, $k_0(\bfx,\calX) = k_0(\bfx,\calP)E^\top$, $E^\top E = \diag(\bfm)$, and $\bfzeta = (E^\top E)^{-1} E^\top \bfy$. Using these expressions in~\eqref{eq:gp_posterior} leads to:
\begin{equation}
\label{eq:E_gp_posterior}
\begin{aligned}
\mu(\bfx) &= \mu_0(\bfx) + k_0(\bfx, \calP)E^\top (Ek_0(\calP, \calP)E^\top+ \sigma^2 I)^{-1}(\bfy - E\mu_0(\calP)),\\
k(\bfx,\bfx') &=  k_0(\bfx, \bfx') - k_0(\bfx, \calP)E^\top (Ek_0(\calP, \calP)E^\top + \sigma^2 I)^{-1} Ek_0(\calP, \bfx').
\end{aligned}
\end{equation}
An application of the matrix inversion lemma followed by algebraic manipulation shows that $E^\top (Ek_0(\calP, \calP)E^\top + \sigma^2 I)^{-1} = \prl{k_0(\calP, \calP) + \sigma^2 (E^\top E)^{-1}}^{-1} (E^\top E)^{-1}E^\top = Z (E^\top E)^{-1}E^\top$. Replacing this and $\bfzeta = (E^\top E)^{-1} E^\top \bfy$ in~\eqref{eq:E_gp_posterior} shows that the GP distributions of $f(\bfx) | \calX,\bfy$ and $f(\bfx) | \calP, \bfzeta$ are equal.
\end{proof}

Prop.~\ref{prop:gp_compression} allows us to summarize a training set $\calX$, $\bfy$ by keeping the distinct training points $\calP$, the average observation value $\zeta(\bfp)$, and the number of times $m(\bfp)$ that each points $\bfp \in \calP$ has been observed. Given these statistics, the mean function $\mu(\bfx)$ and covariance function $k(\bfx,\bfx')$ of the posterior GP can be obtained according to~\eqref{eq:compressed_gp_posterior} with $\bfzeta := \zeta(\calP)$ and $\bfm := m(\calP)$. This leads to significant computational savings when the training points $\calX$ contain repetitions. We will exploit this compression technique for efficient incremental learning when the same locations are observed multiple times online.



\subsection{Incremental GP Regression}

Suppose now that, instead of a single training set, the data are provided sequentially, i.e., an additional dataset $\tilde{\calD}_t$ of training points $\tilde{\calX}_t$ with labels $\tilde{\bfy}_t$ is provided at each time step $t$ so that the cumulative data up to time $t$ are $\calD_t := \cup_{\tau = 1}^t \tilde{\calD}_\tau$. Based on Prop.~\ref{prop:gp_compression}, we can define an incrementally growing set of pseudo inputs $\calP_t$ with associated number of observations $m_t(\bfp)$ and average observation $\zeta_t(\bfp)$ for $\bfp \in \calP_t$ and observation precision $Z_t$. We show how to update these statistics when a new dataset $\tilde{\calX}_{t+1}$, $\tilde{\bfy}_{t+1}$ arrives at time $t+1$. Let $\tilde{\calP}_{t+1}$ be the set of unique points in $\tilde{\calX}_{t+1}$ with number of observations $\tilde{m}_{t+1}(\bfp)$ and average observation $\tilde{\zeta}_{t+1}(\bfp)$ for $\bfp \in \tilde{\calP}_{t+1}$. The update of $\calP_t$, $m_t(\bfp)$ and $\zeta_t(\bfp)$ is straightforward:
\begin{equation}
\begin{aligned}
\calP_{t+1} &= \calP_t \cup \tilde{\calP}_{t+1}\\
m_{t+1}(\bfp) &= \begin{cases}
      m_t(\bfp) + \tilde{m}_{t+1}(\bfp), & \text{if } \bfp \in \calP_t,\\
      \tilde{m}_{t+1}(\bfp), & \text{else},
      \end{cases}\\
\zeta_{t+1}(\bfp) &= \begin{cases}
      \frac{1}{m_{t+1}(\bfp)}\prl{m_t(\bfp)\zeta_t(\bfp) + \tilde{m}_{t+1}(\bfp)\tilde{\zeta}_{t+1}(\bfp)}, & \text{if } \bfp \in \calP_t,\\
      \tilde{\zeta}_{t+1}(\bfp), & \text{else}.
      \end{cases}
\end{aligned}
\end{equation}
To update the observation precision $Z_t$, first consider the existing pseudo inputs $\calP_t$. Let $l$ be the index of $\bfp \in \calP_t$ in $Z_t$. Define $\epsilon_l := \frac{\sigma^2}{m_{t+1}(\bfp)} - \frac{\sigma^2}{m_{t}(\bfp)}$, $A_0 := Z_t$, and for $l = 1,\ldots,|\calP_t|$:
\begin{equation}
A_{l+1} = \prl{A_l^{-1} +  \epsilon_l \bfe_l \bfe_l^\top}^{-1} = A_l - \frac{A_l \bfe_l \bfe_l^\top A_l}{\frac{1}{\epsilon_l} + \bfe_l^\top A_l \bfe_l}.
\end{equation}
With some abuse of notation, let $A := A_{|\calP_t|}$ be the observation precision after all $\bfp \in \calP_t$ have been updated. Finally, we update $A$ by introducing the pseudo inputs $\tilde{\calP}_{t+1}\setminus \calP_t$ that have been observed for the first time:
\begin{equation}
Z_{t+1} = \begin{bmatrix} A^{-1} & B\\ B^\top & D \end{bmatrix}^{-1} = \begin{bmatrix} A + ABSB^\top A & -ABS\\ -S B^\top A & S \end{bmatrix},
\end{equation}
where $B := k_0(\calP_t,\tilde{\calP}_{t+1}\setminus \calP_t)$, $D := k_0(\tilde{\calP}_{t+1}\setminus \calP_t,\tilde{\calP}_{t+1}\setminus \calP_t) + \sigma^2 \diag(\tilde{m}_{t+1}(\tilde{\calP}_{t+1}\setminus \calP_t))^{-1}$, and $S := (D  - B^\top A B)^{-1}$.





\section{Probabilistic Metric-Semantic Mapping}

\subsection{Training Set Construction}

\subsection{Semantic Category Prediction}

\subsection{Octree of Gaussian Processes}




\section{Distributed Incremental GP Regression}
In the sparse GP formulation with pseudo inputs in~\eqref{eq:pseudopoint_gp_posterior}, the posterior is determined by the pseudo input mean and covariance in~\eqref{eq:pseudopoint_distribution}. This section develops a distributed GP formulation by relying on distributed Gaussian filtering techniques to obtain the mean and covariance of the pseudo inputs.

\subsection{Distributed Gaussian Inference}
\TODO{Review Results from CDC14 here}


\subsection{Distributed Incremental GP Regression}

Each robot $k$ receives local data $\tilde{\calX}_t^k$, $\tilde{\bfy}_t^k$ sequentially and maintains a Gaussian density $p(\bff_t^k | \Theta_t^k)$ with the parameters $\Theta_t^k := (\calP_t^k, \bfm_t^k, \bfzeta_t^k, Z_t^k)$ over the latent function value $\bff_t^k := f(\calP_t^k)$  at the pseudo inputs $\calP_t^k$. The parameters $\Theta_t^k$ are sufficient to specify the mean and covariance of $\bff_t^k$:
\begin{equation}
\begin{aligned}
\bfmu_t^k &= \mu_0(\calP_t^k) + k_0(\calP_t^k,\calP_t^k)Z_t^k\prl{\bfzeta_t^k-\mu_0(\calP_t^k) }\\
\Sigma_t^k &=  k_0(\calP_t^k,\calP_t^k) - k_0(\calP_t^k,\calP_t^k)Z_t^k k_0(\calP_t^k,\calP_t^k)
\end{aligned}
\end{equation}
or equivalently the pseudo input information mean and information matrix:
\begin{equation}
\begin{aligned}
\bfomega_t^k &= k_0(\calP_t^k,\calP_t^k)^{-1}\mu_0(\calP_t^k) + \frac{1}{\sigma^2}\diag(\bfm_t^k)\bfzeta_t^k\\
\Omega_t^k &= k_0(\calP_t^k,\calP_t^k)^{-1} + \frac{1}{\sigma^2}\diag(\bfm_t^k)
\end{aligned}
\end{equation}



%\begin{equation}
%\label{eq:pseudopoint_information_distribution}
%\begin{aligned}
%\bfomega &:= \Sigma^{-1}\bfmu = \Omega\mu_0(\calP) + k_0(\calP,\calP)^{-1} k_0(\calP, \calX)\prl{\Lambda + \sigma^2 I}^{-1}(\bfy - \mu_0(\calX))\\
%\Omega &:= \Sigma^{-1} = k_0(\calP,\calP)^{-1} \prl{k_0(\calP,\calP) + \Gamma} k_0(\calP,\calP)^{-1}
%\end{aligned}
%\end{equation}
%With repeated data these simplify to:
%\begin{equation}
%\begin{aligned}
%\bfomega &= k_0(\calP,\calP)^{-1}\mu_0(\calP) + \frac{1}{\sigma^2}\diag(m(\calP))\zeta(\calP)\\
%\Omega &= k_0(\calP,\calP)^{-1} + \frac{1}{\sigma^2}\diag(m(\calP))
%\end{aligned}
%\end{equation}


%\begin{equation}
%\begin{aligned}
%\bfomega &= k_0(\calP,\calP)^{-1}\mu_0(\calP) + \frac{1}{\sigma^2}E^\top\bfy\\
%\Omega &= k_0(\calP,\calP)^{-1} + \frac{1}{\sigma^2}E^\top E
%\end{aligned}
%\end{equation}


\section{Distributed Metric-Semantic Mapping}





==> tex/Sparse.tex <==
%!TEX root = ../main.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% SECTION : Introduction   %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Sparse Gaussian Process Regression}
\label{sec:sparse}

As we have mentioned previously the set of pseudo points and $\bbgamma, \Gamma$ have the inference of the GP. Sometimes cardinal of $\calX_\#$ is infinite or is unnecessarily huge. To address that we do not consider all of the pseudo points, but we consider the growing set of pseudo points $\calX_t \subset \calX_\#$ that capture almost all of the inference, but the cardinality of pseudo points is small.   

\begin{equation}
\label{eq:growGamma}
\begin{aligned}
%
\bbgamma_t &:= k(\calX_t,X_t)(\Lambda_t+\sigma^2I)^{-1}\bby_t\\
%
\Gamma_t &:= k(\calX_t,X_t)(\Lambda_t+\sigma^2I)^{-1}k(X_t, \calX_t)
%
\end{aligned}
\end{equation}

where $X_t, \bby_t$ are data up to time $t$, and $\Lambda_t$ is diagonal matrix builded with function $\lambda(.)$ based on assuming pseudo points to be $\calX_t$. Note that when $\calX_t$ reaches to $\calX_\#$ then we have exactly as we had before.

For example let assume the function that we want to learn is $f(x)=\sin(x) \ \ 0 \leq x \leq \pi$ and $\calX_\# = \{\frac{\pi i}{50}|i\leq 100\}$. Let $\calX_t=\{\frac{20\pi i}{50}|i< 5\}, \bby_t$  be data up to time $t$ such that for any $x \in \calX_t$ its corresponding $y$ in $\bby_t$ is produced due to $y=sin(x)+\epsilon \ \ \epsilon\sim \calN(0,\sigma^2)$.
    
Let in the time $t+1$ we observe $x_{t+1}=\frac{100\pi}{50}, y_{t+1} = 0.001$.

If we use the traditional way and consider all the pseudo points $\calX_\#$ then:

\begin{equation}
\begin{aligned}
%
\bbgamma_t &:= k(\calX_\#,X_t)(\Lambda_t+\sigma^2I)^{-1}\bby_t\\
\bbgamma_{t+1} &:= k(\calX_\#,X_t\cup \{x_{t+1}\})(\Lambda_t+\sigma^2I)^{-1}\bby_{t+1}
%
\end{aligned}
\end{equation}

If we use new method since here $\calX_t=X_t,\calX_{t+1}=X_{t+1}$ we have:

\begin{equation}
\begin{aligned}
%
\bbgamma_t &:= k(X_t,X_t)(\Lambda_t+\sigma^2I)^{-1}\bby_t\\
\bbgamma_{t+1} &:= k(X_t\cup \{x_{t+1}\},X_t\cup \{x_{t+1}\})(\Lambda_t+\sigma^2I)^{-1}\bby_{t+1}
%
\end{aligned}
\end{equation}

\begin{figure}[t]
\includegraphics[width=0.49\columnwidth]{fig/sin4.png}
\includegraphics[width=0.49\columnwidth]{fig/sin2.png}\\
\includegraphics[width=0.49\columnwidth]{fig/sin3.png}
\includegraphics[width=0.49\columnwidth]{fig/sin1.png}
\caption{Comparison between the performance of fixed pseudo points and growing pseudo points, and using Gaussian Process, in which we see in our case they are the same.\TODO{The caption and the figures do not provide sufficient information to distinguish what is going on in the three (blue, red, green) curves. We should show the covariance in addition to the mean and somehow, e.g., using several plots, illustrate how the pseudopoints are growing.}}
\end{figure}

\subsubsection{Equivalence to Gaussian Process}
Since we should consider the effect of previous data on the new pseudo points we should keep all data, which is not efficient. One immediate solution is to do another approximation and ignore the effect of previous data on new pseudo points, but in here that is not our case. Here, a spacial case happens, that is when the data is out of possible pseudo points (repetition could happen). We just need to keep two number for each point in $\calX_t$ as the mean and number of repetition of distinct points. In this regard let see its equivalent Gaussian Process. By equivalent we mean their predictive distribution for a single test point is the same.

Let $K_t=k(\calX_t,\calX_t)$. We see that the predictive distribution for single test point that we can get through Eq.~\ref{eq:pseudoEstimate} (here set of pseudo points is $\calX_t$ instead of $\calX_\#$) is equivalent with the predictive distribution of a Gaussian Process regression when the data is observation at points $\calX_t$ with their observation value to be $K_t\Gamma_t^{-1}\bbgamma_t$ with variance observation $\diag(K_t\Gamma_t^{-1}K_t)$. 

For example when we have one robot, we set growing pseudo points $\calX_t$ to be the distinct points out of $X_t$. Let $|\calX_t| = l$ and $m_1, ... , m_l$ be number of times that each element of $\calX_t$ is repeated in $X_t$, let $D_t = \diag(\frac{\sigma^2}{m_1}, ... , \frac{\sigma^2}{m_l})$, and let $\bbzeta_t$ be the average of observation for each point in $\calX_t$ ($|\calX_t| = |\bbzeta_t|$). Note that based on definition of $\calX_t$, all $m_i$ are nonzero. Additionally, based on pseudo points to be $\calX_t$, then for any point $\bbx \in X_t$ we have that $\lambda(\bbx)=0$.

\begin{equation}
\begin{aligned}
%
K_t^{-1} \Gamma_t K_t^{-1} &= \diag(\frac{m_1}{\sigma^2}, ... , \frac{m_l}{\sigma^2}) = D_t^{-1}\\
K_t\Gamma_t^{-1}\bbgamma_t &= (K_t^{-1}\Gamma_t K_t^{-1})^{-1} K_t^{-1}\bbgamma_t \\
& =  D_t D_t^{-1}\bbzeta_t = \bbzeta_t
%
\end{aligned}
\end{equation}
%
Then in general, we can rewrite simplify $(K_t+\Gamma_t)^{-1}\bbgamma_t $ as:
%
\begin{equation}
\begin{aligned}   
&= (K_t + K_t K_t^{-1} \Gamma_t K_t^{-1} K_t)^{-1}\bbgamma_t\\
&= (K_t + K_t D_t^{-1} K_t)^{-1}\bbgamma_t\\
&= (K_t + K_t D_t^{-1} K_t)^{-1}(D_t K_t^{-1})^{-1}D_t K_t^{-1}\bbgamma_t\\
&= (D_t+ K_t)^{-1} \bbzeta_t\\
%
\end{aligned}
\end{equation}  
and, simplify $K_t^{-1} - (K_t+\Gamma_t)^{-1} $ as:
\begin{equation}
%\scaleMathLine{
\begin{aligned} 
%
&= K_t^{-1} - (K_t + K_t K_t^{-1} \Gamma_t K_t^{-1} K_t)^{-1}\\
&= K_t^{-1} - (K_t + K_t D_t^{-1} K_t)^{-1}\\
&= K_t^{-1} - (K_t^{-1} - K_t^{-1}K_t(D_t + K_tK_t^{-1}K_t)^{-1}K_tK_t^{-1})\\
&= (D_t + K_t)^{-1}
\end{aligned}
%}
\end{equation}  
To see the equivalence with GP we mentioned, we just need to replace the previous equalities in Eq.~\ref{eq:pseudoEstimate}:
\begin{equation}
\scaleMathLine{\begin{aligned}   
\mu_* & = k(\bbx_*, \calX_t) (K_t+\Gamma_t)^{-1}\bbgamma_t = k(\bbx_*, \calX_t) (D_t+ K_t)^{-1} \bbzeta_t \\
\sigma_*^2 & = k(\bbx_*, \bbx_*) - k(\bbx_*, \calX_t)(K_t^{-1} - (K_t+\Gamma_t)^{-1})k(\calX_t, \bbx_*) \\
& = k(\bbx_*, \bbx_*) - k(\bbx_*, \calX_t)(D_t + K_t)^{-1}k(\calX_t, \bbx_*)
\end{aligned}}
\end{equation}   

 then we just need to  keep mean and number of repetition of distinct points. We will see general case in the Prop.~\ref{prop:main1}.


==> tex/SparseGPreg.tex <==
%!TEX root = ../main.tex

%\section{Incremental Bayesian Inference}
%
\section{Sparse Gaussian Process Regression}
\label{sec:sparseGPreg}
A \emph{Gaussian Process} (GP) is a set of random variables such that the joint distribution of any finite subset of them is Gaussian. A GP-distributed function $f(\bfx) \sim \mathcal{GP}(\mu_0(\bfx), k_0(\bfx, \bfx'))$ is defined by a mean function $\mu_0(\bfx)$ and a covariance (kernel) function $k_0(\bfx, \bfx')$. The mean and covariance are such that for any finite set $\calX = \crl{\bfx_1,\ldots,\bfx_M}$, the random vector $f(\calX) := \brl{f(\bfx_1),\ldots,f(\bfx_M)}^\top \in \mathbb{R}^{M}$ has mean with $j$-th element $\mu_0(\bfx_j)$ and covariance matrix with $(j,l)$-th element $k_0(\bfx_j, \bfx_l)$ for $j,l = 1,\ldots,M$. Given a training set $\calD=\{(\bfx_j, y_j)\}_{j=1}^M$, generated according to $y_j=f(\bfx_j)+\epsilon_j$ with independent Gaussian noise $\epsilon_j \sim \calN(0, \sigma^2)$, the posterior distribution of the random function $f(\bfx)$ can be obtained from the joint distribution of the value $f(\bfx)$ at an arbitrary location $\bfx$ and the random vector $\bfy := \brl{y_1,\ldots,y_M}^\top$ of measurements. In detail, the joint distribution is:
\begin{equation}
\begin{aligned}
\begin{bmatrix} f(\bfx) \\ \bfy \end{bmatrix} \sim \mathcal{N}\prl{ \begin{bmatrix} \mu_0(\bfx) \\ \mu_0(\calX) \end{bmatrix}, \begin{bmatrix} k_0(\bfx,\bfx) & k_0(\bfx, \calX)\\
k_0(\calX,\bfx) & k_0(\calX,\calX) + \sigma^2 I\end{bmatrix}},
\end{aligned}
\end{equation}
while the corresponding conditional distribution $f(\bfx)|\calD \sim \mathcal{GP}(\mu(\bfx), k(\bfx, \bfx'))$ has mean and covariance functions:
%
\begin{equation}
\label{eq:gp_posterior}
\scaleMathLine{\begin{aligned}
\mu(\bfx) &:= \mu_0(\bfx) + k_0(\bfx, \calX) (k_0(\calX, \calX)+ \sigma^2 I)^{-1}(\bfy - \mu_0(\calX)),\\
k(\bfx,\bfx') &:=  k_0(\bfx, \bfx') - k_0(\bfx, \calX) (k_0(\calX, \calX) + \sigma^2 I)^{-1} k_0(\calX, \bfx').
\end{aligned}}
\end{equation}
%
Computing the GP posterior has cubic complexity in the number of observations $M$ due to the matrix inversion in~\eqref{eq:gp_posterior}.


Inspired by Snelson and Ghahramani~\cite{snelson2006sparse}, we introduce a sparse approximation to the GP posterior in~\eqref{eq:gp_posterior} using a set of \emph{pseudo points} $\calP\subset \calD$ whose number $|\calP| \ll M$. The key idea is to first determine the distribution $\calN\prl{\bfmu,\Sigma}$ of $\bff := f(\calP)$ conditioned on $\calX$, $\bfy$ according to~\eqref{eq:gp_posterior}:
%
\begin{align}\label{eq:pseudopoint_distribution}
\bfmu &:= \mu_0(\calP) + k_0(\calP, \calX) (k_0(\calX, \calX)+ \sigma^2 I)^{-1}(\bfy - \mu_0(\calX))\notag\\
 &\phantom{:}= \mu_0(\calP)+k_0(\calP,\calP)\prl{k_0(\calP,\calP) + \Gamma}^{-1}\bbgamma\\ 
\Sigma &:=  k_0(\calP,\calP) - k_0(\calP,\calX)\prl{ k_0(\calX,\calX) + \sigma^2 I }^{-1} k_0(\calX,\calP),\notag\\
 &\phantom{:}= k_0(\calP,\calP)\prl{k_0(\calP,\calP) + \Gamma}^{-1}k_0(\calP,\calP)\notag
\end{align}
%
where $\Gamma := k_0(\calP,\calX)\prl{\Lambda + \sigma^2 I}^{-1}k_0(\calX,\calP)$, $\Lambda := k_0(\calX,\calX) - k_0(\calX,\calP) k_0(\calP,\calP)^{-1} k_0(\calP,\calX)$, and $\bbgamma := k_0(\calP,\calX)\prl{\Lambda + \sigma^2 I}^{-1}(\bfy - \mu_0(\calX))$. 
%where $\Lambda(X_n)$ is a diagonal matrix with entries $\lambda(\bfx_j) := k_0(\bfx_j,\bfx_j) - k_0(\bfx_j,P_n)k_0(P_n,P_n)^{-1} k_0(P_n,\bfx_j)$ on the diagonal.
Then, the posterior of $f(\bfx)$ conditioned on $\calX, \bfy$ is:
\begin{equation}
p( f(\bfx) | \calX, \bfy) = \int p(f(\bfx) | \bff) p(\bff | \calX, \bfy) d\bff
\end{equation}
which is a GP with mean and covariance functions:
\begin{equation}
\label{eq:pseudopoint_gp_posterior}
\begin{aligned}
\mu(\bfx)% &= \mu_0(\bfx) + k_0(\bfx, \calP)k_0(\calP,\calP)^{-1}\prl{\bfmu - \mu_0(\calP)}\\
&=\mu_0(\bfx) + k_0(\bfx, \calP)\prl{k_0(\calP,\calP) + \Gamma}^{-1}\bbgamma\\
k(\bfx,\bfx') %&= k_0(\bfx,\calP) k_0(\calP,\calP)^{-1}\Sigma k_0(\calP,\calP)^{-1} k_0(\calP,\bfx')\\ 
%&\quad + k_0(\bfx,\bfx') - k_0(\bfx,\calP)k_0(\calP,\calP)^{-1}k_0(\calP,\bfx')\\
&=k_0(\bfx,\calP) \prl{k_0(\calP,\calP) + \Gamma}^{-1} k_0(\calP,\bfx')\\ 
&\quad + k_0(\bfx,\bfx') - k_0(\bfx,\calP)k_0(\calP,\calP)^{-1}k_0(\calP,\bfx').
\end{aligned}
\end{equation}
where $\Gamma$ and $\bbgamma$ are defined above.
If we assume that conditioned on $\calP$, the measurements $y_j$ are generated independently, i.e., $\Lambda$ is approximated by a diagonal matrix with elements $\lambda(\bfx_j) := k_0(\bfx_j,\bfx_j) - k_0(\bfx_j,\calP)k_0(\calP,\calP)^{-1}k_0(\calP,\bfx_j)$, then the complexity of computing $\bfmu$, $\Sigma$ in~\eqref{eq:pseudopoint_distribution} (training) and $\mu(\bfx)$, $k(\bfx,\bfx')$ in~\eqref{eq:pseudopoint_gp_posterior} (testing) are $O(|\calP|^2 |\calX| + |\calP|^3)$ and $O(|\calP|^2)$, respectively, instead of $O(|\calX|^3)$ and $O(|\calX|^2)$ without pseudo points in~\eqref{eq:gp_posterior}. The use of pseudo points leads to significant computational savings when $|\calP| \ll |\calX|$. %\blue{Overall it is good, but this insight that is presented here is our insight, it is not the idea in Snelson and Ghahramani~\cite{snelson2006sparse}, all the idea they have was to assume that having the assuming all the inference of GP in the pseudo points, so in their method you could not calculate mutual covariance in \eqref{eq:pseudopoint_gp_posterior}, so technically the posterior of their model is not a GP, it is just an approximation for the distribution of single test point in real GP. I suggest either we do not mention Snelson and Ghahramani~\cite{snelson2006sparse} or say something general like "inspired from ...." make this point clear.}


==> tex/background.tex <==
%!TEX root = ../main.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% SECTION : Introduction   %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Gaussian Process Regression}
\label{sec:background}

A \emph{Gaussian Process} (GP) is a set of random variables such that the joint distribution of any finite subset of them is Gaussian. A GP-distributed function $f(\bfx) \sim \mathcal{GP}(\mu_0(\bbx), k_0(\bbx, \bbx'))$ is defined by a mean function $\mu_0(\bfx)$ and a covariance (kernel) function $k_0(\bbx, \bbx')$. The mean and covariance are such that for any finite set $X = \crl{\bfx_1,\ldots,\bfx_n}$, the random vector $f(X) := \brl{f(\bfx_1),\ldots,f(\bfx_n)}^\top \in \mathbb{R}^{n}$ has mean with $j$-th element $\mu_0(\bfx_j)$ and covariance matrix with $(j,k)$-th element $k_0(\bbx_j, \bbx_k)$ for $j,k = 1,\ldots,K$. Given a training dataset $\setD=\{(\bfx_j, y_j)\}_{j=1}^n$ generated according to $y_j=f(\bbx_j)+\epsilon_j$ with noise $\epsilon_j \sim \calN(0, \sigma_j^2)$, the posterior distribution of the random function $f(\bfx)$ can be obtained from the joint distribution of the value $f(\bfx)$ at an arbitrary location $\bfx$ and the random vector $\bfy := \brl{y_1,\ldots,y_n}^\top$ of measurements. In detail, the joint distribution is:
\begin{equation}
\scaleMathLine[0.9]{\begin{aligned}
\begin{bmatrix} f(\bfx) \\ \bfy \end{bmatrix} \sim \mathcal{N}\prl{ \begin{bmatrix} \mu_0(\bfx) \\ \mu_0(X) \end{bmatrix}, \begin{bmatrix} k_0(\bfx,\bfx) & k_0(\bfx, X)\\
k_0(X,\bfx) & k_0(X,X) + D\end{bmatrix}},
\end{aligned}}
\end{equation}
where $D \in \mathbb{R}^{n\times n}$ is a diagonal matrix with $D_{i,i} = \sigma_i^2$, while the corresponding conditional distribution $f(\bbx)|\setD \sim \mathcal{GP}(\mu_n(\bbx), k_n(\bbx, \bbx'))$ has mean and covariance functions:
%
\begin{equation*}
\scaleMathLine{\begin{aligned}
\mu_n(\bfx) &= \mu_0(\bfx) + k_0(\bfx, X) (k_0(X, X)+ D)^{-1}(\bby - \mu_0(X)),\\
k_n(\bfx,\bfx') &=  k_0(\bfx, \bfx') - k_0(\bfx, X) (k_0(X, X)+D)^{-1} k_0(X, \bfx').
\end{aligned}}
\end{equation*}
%
Computing the GP posterior has cubic complexity in the number of observations $n$ due to the $n \times n$ matrix inversion.
%
%
%
%

In order to deal with the cubic complexity of Gaussian Process \cite{snelson2006sparse}, suggests assuming existence of a pseudo data with smaller size than the real data set, but the distribution estimation of both are very close. In this case we can say that the inference by both data sets are the same, so the pseudo data set is the sufficient statistics for the GP that is built based on the real data set. Hence, we can build our GP based on this pseudo data set instead of real data set. The sparsity arises from the fact that size of pseudo data set is smaller than the real one.

We have $\calX_\#$ as set of all pseudo points, with their latent values $\bbf_\#=f(\calX_\#)$. We assume these pseudo points are enough to train the GP, so given $\calX_\#, \bbf_\#$ the distribution of observation at different points are independent of each other. As it is calculated in \cite{snelson2006sparse}  for specific point $\bbx$ the distribution is\NA{Using the symbol $\calN$ for the Gaussian probability density function is not recommended because it can easily be confused with the Gaussian distribution} \blue{Inspired by people's use, I have used $\mathcal{GP}$ for GP, $\calN(\mu,\sigma^2)$ for normal distribution, and $\calN(y|\mu,\sigma^2)$, I could not think of better notation. Please let me know if you think there is better one. }:
%
\begin{equation*}
%\scaleMathLine{
\begin{aligned}
%
p(y| \bbf_\#) = \calN(y|k(\bbx, \calX_\#){K_\#}^{-1}\bbf_\#,\lambda(\bbx)+\sigma^2)
%
\end{aligned}
%}
\end{equation*}
%
where $K_\# = k(\calX_\#, \calX_\#)$, and $\lambda(\bbx) = k(\bbx,\bbx)-k(\bbx, \calX_\#){K_\#}^{-1}k(\calX_\#,\bbx)$, or equivalently we can say:
%
\begin{equation}
\begin{aligned}
%
y = & k(\bbx, \calX_\#){K_\#}^{-1}\bbf_\# +\epsilon(\bbx), \\
&\epsilon(\bbx) \sim \calN(0, \lambda(\bbx)+\sigma^2)
%
\end{aligned}
\end{equation}
%

Hence observing measurements values $Y=\{y_1,...,y_n\}$ at locations $X=\{\bbx_1,...,\bbx_n\}$ as dataset, the assumption lies in the sufficient statistics being value of function on $\calX_\#$ is the i.i.d. nature of the dataset given the function on the $\calX_\#$, i.e.:

\begin{equation}
\begin{aligned}
&p(\bby|\bbf_\#) = \prod_{i=1}^n p(y_i | \bbf_\#) \\ %p(y_i|\bbx_i, \bbf_\#, \calX_\#)
&= \calN(\bby | k(X, \calX_\#){K_\#}^{-1}\bbf_\#, \Lambda+\sigma^2 I)
\end{aligned}
\end{equation}
where $\Lambda = \diag(\lambda(\bbx_1), ..., \lambda(\bbx_n))$. Define:

\begin{equation}
\label{Def:gamma}
\begin{aligned}
%
\bbgamma &:= k(\calX_\#,X)(\Lambda+\sigma^2I)^{-1}\bby\\
%
\Gamma &:= k(\calX_\#,X)(\Lambda+\sigma^2I)^{-1}k(X, \calX_\#)
%
\end{aligned}
\end{equation}

 Then if we place a prior $p(\bbf_\#) = \calN(\bbf_\# | \bb0, K_\#)$ on the pseudo points, then by Bayes rule we have the posterior:

\begin{equation}
\label{eq:posterior}
\begin{aligned}
p(\bbf_\# | \bby) = \calN(\bbf_\# | K_\#{(K_\#+\Gamma)}^{-1}\bbgamma,  K_\#( K_\#+\Gamma)^{-1} K_\#)
\end{aligned}
\end{equation}

In order to calculate predictive distribution of latent function $f_*$ at some point $\bbx_*$, note that given $\bbf_\#$ we assumed other points are independent of each other (this means joint distribution of several points does not have meaning and evaluation of one point is meaningful under these assumptions), so having $p(\bbf_\# | \bby)$ we can calculate:
 
\begin{equation}
\label{eq:pseudoEstimate}
\scaleMathLine{\begin{aligned}   
p(f_* | \bby) &= \int p(f_* | \bbf_\#) p(\bbf_\# | \bby) \bbd \bbf_\# = \calN(f_* | \mu_*, \sigma_*^2)\\
\mu_* & = k(\bbx_*, \calX_\#) (K_\#+\Gamma)^{-1}\bbgamma \\
\sigma_*^2 & = k(\bbx_*, \bbx_*) - k(\bbx_*, \calX_\#)(K_\#^{-1} - (K_\#+\Gamma)^{-1})k(\calX_\#, \bbx_*)
\end{aligned}}
\end{equation}   

As we can see having $\Gamma, \bbgamma$ and $\calX_\#$ are sufficient to calculate the predictive distribution of latent function on single points in the continuous environment. 
%we need to keep track of distribution of $\bbf_\#|X,Y \sim \calN(\Omega^{-1}\omega, \Omega^{-1})$: 

%------------------------------------------------------------------------------------------------------------------------------------------------------------------
%
%\begin{equation}
%\begin{aligned}
%
%\bbomega &= k(\calX_\#, \calX_\#)^{-1}k(\calX_\#,X)(\Lambda+\sigma^2I)^{-1}\bby\\
%
%\Omega &= k(\calX_\#, \calX_\#)^{-1} + k(\calX_\#, \calX_\#)^{-1}\\
%&k(\calX_\#,X)(\Lambda+\sigma^2I)^{-1}k(X, \calX_\#)k(\calX_\#, \calX_\#)^{-1}
%
%\end{aligned}
%\end{equation}

%Let define:

%\begin{equation}
%\label{eq:gamma}
%\begin{aligned}
%
%\bbgamma &:= k(\calX_\#,X)(\Lambda+\sigma^2I)^{-1}\bby\\
%
%\Gamma &:= k(\calX_\#,X)(\Lambda+\sigma^2I)^{-1}k(X, \calX_\#)
%
%\end{aligned}
%\end{equation}

%Then we have:
 
%\begin{equation}
%\label{eq:mu}
%\begin{aligned}
%\bbomega &:= k(\calX_\#, \calX_\#)^{-1}\bbgamma\\
%\Omega &:= k(\calX_\#, \calX_\#)^{-1} (k(\calX_\#, \calX_\#)+\Gamma) k(\calX_\#, \calX_\#)^{-1}\\
%\bbmu &= \Omega^{-1}\bbomega = k(\calX_\#, \calX_\#) (k(\calX_\#, \calX_\#)+\Gamma)^{-1}\bbgamma\\
%\Sigma &= \Omega^{-1} = k(\calX_\#, \calX_\#) (k(\calX_\#, \calX_\#)+\Gamma)^{-1} k(\calX_\#, \calX_\#)
%\end{aligned}
%\end{equation}
%
%

\subsection{Update New Observation}
\label{sec:NewObservation}
For fixed pseudo points $\calX_\#$, in order to update the inference at time $t$ i.e. $\Gamma_{t}, \bbgamma_{t}$ two case might happen. 
First case is observing new observation, for one observation $y_*$ at $\bbx_*$ with regard to Def.~\ref{Def:gamma} we can update $\Gamma_t$ and $\bbgamma_t$:
%
%
%
%
\begin{equation}
\label{dataupdate}
\begin{aligned}
%
\bbgamma_{t+1} &= \bbgamma_{t}+\frac{y_*k(\calX_\#,\bbx_*)}{\lambda(\bbx_*)+\sigma^2}\\
%
\Gamma_{t+1} &= \Gamma_{t}+\frac{k(\calX_\#, \bbx_*)k(\bbx_*, \calX_\#)}{\lambda(\bbx_*)+\sigma^2}
%
\end{aligned}
\end{equation}
%


==> tex/evaluationFigures/classfigure1.tex <==
%!TEX root = ../../main.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% SECTION : Problem   %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htbp]
%\centering
%
%
%
\begin{subfigure}[t]{1\linewidth}
%
%
%
%\centering
\includegraphics[width=8cm]{tex/evaluationFigures/class1}
%
%
%
\caption{The final reconstruction out of $2450$ RGBD images. Number of classes detected is $85$ classes. This reconstruction took $1040.41$ seconds.}
%
%
%
\end{subfigure}\\
%
%
%
\begin{subfigure}[t]{1\linewidth}
%
%
%
%\centering
\includegraphics[width=8cm]{tex/evaluationFigures/class2}
%
%
%
\caption{The final reconstruction out of $3700$ RGBD images. Number of classes detected is $61$ classes. This reconstruction took $1885.72$ seconds.}
%
%
%
\end{subfigure}
%
%
%
%\captionsetup{format=plain, font=small, labelfont=bf}
\caption{$\delta\ =\ 1.5$, $N_\ccalX \ =\ 100$, Gaussian Process noise variance $=\ 3$, Voxel size $=\ 0.03$.}%3D class reconstruction, on the left we see reconstruction of local area, and on the right we see a result over all room.
%
%
%
\end{figure}\label{hihi}
%
%
%
%
%
%

\begin{figure*}[htbp]
\centering
%
%
%
%environment 
%SDF Red class
\begin{subfigure}[t]{0.12\linewidth}
\centering
%
%
%
\includegraphics[width=2.4cm]{tex/evaluationFigures/maxInLeaf/mesh_5}
%
%
%
\caption{$N_\ccalX=5$, $time = 58.15$}
%
%
%
\end{subfigure}
%
%
%
\begin{subfigure}[t]{0.12\linewidth}
%
%
%
\centering
%
%
%
\includegraphics[width=2.4cm]{tex/evaluationFigures/maxInLeaf/mesh_10}
%
%
%
\caption{$N_\ccalX=10$, $time = 49.35$}
%
%
%
\end{subfigure}
%
%
%
\begin{subfigure}[t]{0.12\linewidth}
%
%
%
\centering
%
%
%
\includegraphics[width=2.4cm]{tex/evaluationFigures/maxInLeaf/mesh_50}
%
%
%
\caption{$N_\ccalX=50$, $time = 41.64$}
%
%
%
\end{subfigure}
%
%
%
\begin{subfigure}[t]{0.12\linewidth}
%
%
%
\centering
%
%
%
\includegraphics[width=2.4cm]{tex/evaluationFigures/maxInLeaf/mesh_100}
%
%
%
\caption{$N_\ccalX=100$, $time = 45.15$}
%
%
%
\end{subfigure}
%
%
%
\begin{subfigure}[t]{0.12\linewidth}
%
%
%
\centering
%
%
%
\includegraphics[width=2.4cm]{tex/evaluationFigures/maxInLeaf/mesh_200}
%
%
%
\caption{$N_\ccalX=200$, $time = 47.94$}
%
%
%
\end{subfigure}
%
%
%
\begin{subfigure}[t]{0.12\linewidth}
%
%
%
\centering
%
%
%
\includegraphics[width=2.4cm]{tex/evaluationFigures/maxInLeaf/mesh_1000}
%
%
%
\caption{$N_\ccalX=1000$, $time = 96.83$}
%
%
%
\end{subfigure}\\
%
%
%
%
\begin{subfigure}[t]{0.12\linewidth}
%
%
%
\centering
%
%
%
\includegraphics[width=2.4cm]{tex/evaluationFigures/dimRatio/mesh_1}
%
%
%
\caption{$\delta=1$, $time = 32.62$}
%
%
%
\end{subfigure}
%
%
%
\begin{subfigure}[t]{0.12\linewidth}
%
%
%
\centering
%
%
%
\includegraphics[width=2.4cm]{tex/evaluationFigures/dimRatio/mesh_12}
%
%
%
\caption{$\delta=1.2$, $time = 35.54$}
%
%
%
\end{subfigure}
%
%
%
\begin{subfigure}[t]{0.12\linewidth}
%
%
%
\centering
%
%
%
\includegraphics[width=2.4cm]{tex/evaluationFigures/dimRatio/mesh_14}
%
%
%
\caption{$\delta=1.4$, $time = 39.11$}
%
%
%
\end{subfigure}
%
%
%
\begin{subfigure}[t]{0.12\linewidth}
%
%
%
\centering
%
%
%
\includegraphics[width=2.4cm]{tex/evaluationFigures/dimRatio/mesh_16}
%
%
%
\caption{$\delta=1.6$, $time = 44.15$}
%
%
%
\end{subfigure}
%
%
%
\begin{subfigure}[t]{0.12\linewidth}
%
%
%
\centering
%
%
%
\includegraphics[width=2.4cm]{tex/evaluationFigures/dimRatio/mesh_18}
%
%
%
\caption{$\delta=1.8$, $time = 49.44$}
%
%
%
\end{subfigure}
%
%
%
\begin{subfigure}[t]{0.12\linewidth}
%
%
%
\centering
%
%
%
\includegraphics[width=2.4cm]{tex/evaluationFigures/dimRatio/mesh_2}
%
%
%
\caption{$\delta=2$, $time = 57.41$}
%
%
%
\end{subfigure}\\
%
%
%
%
\begin{subfigure}[t]{0.12\linewidth}
%
%
%
\centering
%
%
%
\includegraphics[width=2.4cm]{tex/evaluationFigures/sigma/mesh_0}
%
%
%
\caption{$\sigma=0$, $time = 42.43$}
%
%
%
\end{subfigure}
%
%
%
\begin{subfigure}[t]{0.12\linewidth}
%
%
%
\centering
%
%
%
\includegraphics[width=2.4cm]{tex/evaluationFigures/sigma/mesh_1}
%
%
%
\caption{$\sigma=1$, $time = 45.47$}
%
%
%
\end{subfigure}
%
%
%
\begin{subfigure}[t]{0.12\linewidth}
%
%
%
\centering
%
%
%
\includegraphics[width=2.4cm]{tex/evaluationFigures/sigma/mesh_2}
%
%
%
\caption{$\sigma=2$, $time = 42.43$}
%
%
%
\end{subfigure}
%
%
%
\begin{subfigure}[t]{0.12\linewidth}]%
%
%
\centering
%
%
%
\includegraphics[width=2.4cm]{tex/evaluationFigures/sigma/mesh_10}
%
%
%
\caption{$\sigma=10$, $time = 41.07$}
%
%
%
\end{subfigure}
%
%
%
\begin{subfigure}[t]{0.12\linewidth}
%
%
%
\centering
%
%
%
\includegraphics[width=2.4cm]{tex/evaluationFigures/sigma/mesh_20}
%
%
%
\caption{$\sigma=20$, $time = 42.37$}
%
%
%
\end{subfigure}
%
%
%
\begin{subfigure}[t]{0.12\linewidth}
%
%
%
\centering
%
%
%
\includegraphics[width=2.4cm]{tex/evaluationFigures/sigma/mesh_40}
%
%
%
\caption{$\sigma=40$, $time = 43.76$}
%
%
%
\end{subfigure}\\
%
%
%
%
\begin{subfigure}[t]{0.24\linewidth}
%
%
%
\centering
%
%
%
\includegraphics[width=4.8cm]{tex/evaluationFigures/voxel/mesh_6}
%
%
%
\caption{$voxel=0.06$, $time = 23.24$}
%
%
%
\end{subfigure}
%
%
%
\begin{subfigure}[t]{0.24\linewidth}
%
%
%
\centering
%
%
%
\includegraphics[width=4.8cm]{tex/evaluationFigures/voxel/mesh_3}
%
%
%
\caption{$voxel=0.03$, $time = 45.15$}
%
%
%
\end{subfigure}
%
%
%
\begin{subfigure}[t]{0.24\linewidth}
%
%
%
\centering
%
%
%
\includegraphics[width=4.8cm]{tex/evaluationFigures/voxel/mesh_1}
%
%
%
\caption{$voxel=0.01$, $time = 381.02$}
%
%
%
\end{subfigure}
%
%
%
%
%
%
%\captionsetup{format=plain, font=small, labelfont=bf}
\caption{$\delta\ =\ 1.5$, $N_\ccalX \ =\ 100$, Gaussian Process noise variance $=\ 3$, Voxel size $=\ 0.03$ over $140$ RGBD images.}%3D class reconstruction, on the left we see reconstruction of local area, and on the right we see a result over all room.
%
%
%
\end{figure*}\label{classPara}


==> tex/evaluationFigures/classfigure2.tex <==
%!TEX root = ../../main.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% SECTION : Problem   %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}{0.40\linewidth}
\centering
%
\begin{subfigure}[t]{\linewidth}
%
\includegraphics[width=\linewidth]{tex/evaluationFigures/class1}
%
\caption{The final reconstruction out of $2450$ RGBD images. Number of classes detected is $85$ classes. This reconstruction took $1040.41$ seconds.}
%
\end{subfigure}\\
%
%
\begin{subfigure}[t]{\linewidth}
%
\includegraphics[width=\linewidth]{tex/evaluationFigures/class2}
%
\caption{The final reconstruction out of $3700$ RGBD images. Number of classes detected is $61$ classes. This reconstruction took $1885.72$ seconds.}
%
\end{subfigure}
%
\end{subfigure}
%
%
%
%
%
%
\begin{subfigure}{0.60\linewidth}
%
\begin{subfigure}[t]{0.24\linewidth}
\includegraphics[width=\linewidth]{tex/evaluationFigures/maxInLeaf/mesh_5}
\caption{$N_{Max}=5$, $time = 58.15$}
\end{subfigure}
%
\begin{subfigure}[t]{0.24\linewidth}
\includegraphics[width=\linewidth]{tex/evaluationFigures/maxInLeaf/mesh_50}
\caption{$N_{Max}=50$, $time = 41.64$}
\end{subfigure}
%
\begin{subfigure}[t]{0.24\linewidth}
\includegraphics[width=\linewidth]{tex/evaluationFigures/maxInLeaf/mesh_100}
\caption{$N_{Max}=100$, $time = 45.15$}
\end{subfigure}
%
\begin{subfigure}[t]{0.24\linewidth}
\includegraphics[width=\linewidth]{tex/evaluationFigures/maxInLeaf/mesh_1000}
\caption{$N_{Max}=1000$, $time = 96.83$}
\end{subfigure}\\
%
%
%
%
%
%
\begin{subfigure}[t]{0.24\linewidth}
\includegraphics[width=\linewidth]{tex/evaluationFigures/dimRatio/mesh_1}
\caption{$\delta=1$, $time = 32.62$}
\end{subfigure}
%
\begin{subfigure}[t]{0.24\linewidth}
\includegraphics[width=\linewidth]{tex/evaluationFigures/dimRatio/mesh_12}
\caption{$\delta=1.2$, $time = 35.54$}
\end{subfigure}
%
\begin{subfigure}[t]{0.24\linewidth}
\includegraphics[width=\linewidth]{tex/evaluationFigures/dimRatio/mesh_14}
\caption{$\delta=1.4$, $time = 39.11$}
\end{subfigure}
%
\begin{subfigure}[t]{0.24\linewidth}
\includegraphics[width=\linewidth]{tex/evaluationFigures/dimRatio/mesh_2}
\caption{$\delta=2$, $time = 57.41$}
\end{subfigure}\\
%
%
%
%
%
%
\begin{subfigure}[t]{0.24\linewidth}
\includegraphics[width=\linewidth]{tex/evaluationFigures/sigma/mesh_0}
\caption{$\sigma=0$, $time = 42.43$}
\end{subfigure}
%
\begin{subfigure}[t]{0.24\linewidth}
\includegraphics[width=\linewidth]{tex/evaluationFigures/sigma/mesh_10}
\caption{$\sigma=10$, $time = 41.07$}
\end{subfigure}
%
\begin{subfigure}[t]{0.24\linewidth}
\includegraphics[width=\linewidth]{tex/evaluationFigures/sigma/mesh_20}
\caption{$\sigma=20$, $time = 42.37$}
\end{subfigure}
%
\begin{subfigure}[t]{0.24\linewidth}
\includegraphics[width=\linewidth]{tex/evaluationFigures/sigma/mesh_40}
\caption{$\sigma=40$, $time = 43.76$}
\end{subfigure}\\
%
%
%
%
%
%
\begin{subfigure}[t]{0.24\linewidth}
\includegraphics[width=\linewidth]{tex/evaluationFigures/voxel/mesh_6}
\caption{$voxel=0.06$, $time = 23.24$}
\end{subfigure}
%
\begin{subfigure}[t]{0.24\linewidth}
\includegraphics[width=\linewidth]{tex/evaluationFigures/voxel/mesh_3}
\caption{$voxel=0.03$, $time = 45.15$}
\end{subfigure}
%
\begin{subfigure}[t]{0.24\linewidth}
\includegraphics[width=\linewidth]{tex/evaluationFigures/voxel/mesh_1}
\caption{$voxel=0.01$, $time = 381.02$}
\end{subfigure}
%
\begin{subfigure}[t]{0.24\linewidth}
\includegraphics[width=\linewidth]{tex/evaluationFigures/voxel/mesh_1}
\caption{$voxel=0.01$, $time = 381.02$}
\end{subfigure}
%
\caption{Over $140$ RGBD images.}
\end{subfigure}
\caption{The default parameters are $\delta\ =\ 1.5$, $N_{Max} \ =\ 100$, Gaussian Process noise variance $=\ 3$, Voxel size $=\ 0.03$, frame size $=\ 1$.}
%

==> tex/evaluationFigures/classfigure3.tex <==
%!TEX root = ../../main.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% SECTION : Problem   %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}{0.373\linewidth}
\centering
%
\begin{subfigure}[t]{\linewidth}
%
\includegraphics[width = \linewidth]{tex/evaluationFigures/class1}
%
%\caption{The final reconstruction out of $2450$ RGBD images. Number of classes detected is $85$ classes. This reconstruction took $1040.41$ seconds.}
%
\end{subfigure}\\
%
%
\begin{subfigure}[t]{\linewidth}
%
\includegraphics[width=\linewidth]{tex/evaluationFigures/class2}
%
%\caption{The final reconstruction out of $3700$ RGBD images. Number of classes detected is $61$ classes. This reconstruction took $1885.72$ seconds.}
%
\end{subfigure}
%
\end{subfigure}
%
%
%
%
\begin{subfigure}{0.627\linewidth}
%
\begin{subfigure}[t]{0.24\linewidth}
\includegraphics[width=\linewidth]{tex/evaluationFigures/maxInLeaf/mesh_5}
\caption{\scriptsize$n:5$,$t:58.15$}
\end{subfigure}
%
\begin{subfigure}[t]{0.24\linewidth}
\includegraphics[width=\linewidth]{tex/evaluationFigures/dimRatio/mesh_1}
\caption{\scriptsize$\delta:1,t:32.62$}
\end{subfigure}
%
\begin{subfigure}[t]{0.24\linewidth}
\includegraphics[width=\linewidth]{tex/evaluationFigures/sigma/mesh_0}
\caption{\scriptsize$\sigma^2:0,t:42.43$}
\end{subfigure}
%
\begin{subfigure}[t]{0.24\linewidth}
\includegraphics[width=\linewidth]{tex/evaluationFigures/voxel/mesh_6}
\caption{\scriptsize$v:0.06,t:23.24$}
\end{subfigure}\\
%
%
%
\begin{subfigure}[t]{0.24\linewidth}
\includegraphics[width=\linewidth]{tex/evaluationFigures/maxInLeaf/mesh_100}
\caption{\scriptsize$n:100$,$t:45.15$}
\end{subfigure}
%
\begin{subfigure}[t]{0.24\linewidth}
\includegraphics[width=\linewidth]{tex/evaluationFigures/dimRatio/mesh_14}
\caption{\scriptsize$\delta:1.4,t:39.11$}
\end{subfigure}
%
\begin{subfigure}[t]{0.24\linewidth}
\includegraphics[width=\linewidth]{tex/evaluationFigures/sigma/mesh_10}
\caption{\scriptsize$\sigma^2:10,t:41.07$}
\end{subfigure}
%
\begin{subfigure}[t]{0.24\linewidth}
\includegraphics[width=\linewidth]{tex/evaluationFigures/voxel/mesh_3}
\caption{\scriptsize$v:0.03,t:45.15$}
\end{subfigure}\\
%
%
%
\begin{subfigure}[t]{0.24\linewidth}
\includegraphics[width=\linewidth]{tex/evaluationFigures/maxInLeaf/mesh_1000}
\caption{\scriptsize$n:1000$,$t:96.83$}
\end{subfigure}
%
\begin{subfigure}[t]{0.24\linewidth}
\includegraphics[width=\linewidth]{tex/evaluationFigures/dimRatio/mesh_2}
\caption{\scriptsize$\delta:2,t:57.41$}
\end{subfigure}
%
\begin{subfigure}[t]{0.24\linewidth}
\includegraphics[width=\linewidth]{tex/evaluationFigures/sigma/mesh_40}
\caption{\scriptsize$\sigma^2:40,t:43.76$}
\end{subfigure}
%
\begin{subfigure}[t]{0.24\linewidth}
\includegraphics[width=\linewidth]{tex/evaluationFigures/voxel/mesh_1}
\caption{\scriptsize$v:0.01,t:381.02$}
\end{subfigure}
\end{subfigure}
%------------------------------------------------------------------------------------------------------------------------------------------------------------------
%
%
%\caption{Over $140$ RGBD images.}
%
%
%
\caption{The default parameters are $\delta\ =\ 1.5$, $N_{Max} (n)\ =\ 100$, Gaussian Process noise variance $(\sigma^2)=\ 3$, $voxel\ size\ =\ 0.03$, $frame\ size\ =\ 1$.On the right we see the change of parameters over $140$ RGBD images ($t$ is time in seconds). Left up is the final reconstruction out of $2450$ RGBD images. Number of classes detected is $85$ classes. This reconstruction took $1040.41$ seconds. Left down is the final reconstruction out of $3700$ RGBD images. Number of classes detected is $61$ classes. This reconstruction took $1885.72$ seconds. On the right we see the change of parameters over $140$ RGBD images.}
%

==> tex/gpblock.tex <==
%!TEX root = ../main.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% SECTION : Introduction   %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Sparse Probabilistic Mapping}
%
%
%
%
%
%
\subsection{Gaussian Process Regression}
%
As explained in Appendix~\ref{class}, for simplicity, we assume the covariance kernel of points in different classes are zero, which amounts to $N$ independent Gaussian Processes $f_c$ for each class $c$. In particular, at each time step $t$, we seek to infer the posterior distribution $\mathbb{P}(f_c(\cdot)\given\setD_{t,c})$ for training set $\setD_{t,c}$ at time $t$.
%In order to learn $f_c$, objective signed distance function, from \textcolor{blue}{recap what are the features right here}, we adopt the framework of Gaussian Processes. In this setup, we hypothesize that $f_c(x)\sim \mathcal{GP}(m(x),k(x,x'))$ is a Gaussian Process.
%
%
%
%
%
%At each time step $t$ we will have sample $\setD_{t,c}$ of this gaussian process. Since we pick the pseudo points in $\setD_{t,c}$ out of $\ccalX_\#$, number of points with distinct locations will not grow with time, and it will stay as complex as the environment's complexity, but we may see each pseudo point several times.If there is no noise in observation several observation of a point does not have any meaning (since they all have to be the same). In Gaussian Process with noise we should consider distinct row and column in covariance matrix for each observation, even if we have several observation of same location. It implies the complexity of Gaussian Process grows with time. Following general theorem about noisy Gaussian Process addresses this problem.
%
%
%
%
%
As the robot navigates and obtains depth and class observations of the environment, the procedure outlined in Sec.~\ref{sec:training_set} is used to generate training data $D_{t,c}$ for each object class $c$. Since the complexity of GP is cubic with number of observations, in order to make GP's complexity proportional to environment's complexity, the training points $\bfx$ were chosen from a set $\calX_{\#}$, many of the signed distance measurements will be associated with the same spatial location $\bfx$. Since the GP in the setting we focus on has observations corrupted by noise, selecting training points out of set $\calX_{\#}$ rather than $\calX$ does not address the scalability challenges alone. However, this training subset definition can be employed to define GP posteriors whose complexity is cubic in the number of distinct observed points from $\calX_{\#}$, rather than the number of observations $\sum_t |D_{t,c}|$, which grows unbounded with time. We proceed with a Lemma~\ref{lemma2} that establishes how the parametric updates for GPs change when we merge training points.

\begin{theorem}\label{main1}
Consider $f(\bbx) \sim \mathcal{GP}(m(\bbx),k(\bbx,\bbx'))$. Let: 
%
\begin{equation}
\begin{aligned}
%
X&=\{\bbx_1,\bbx_1,...,\bbx_1,\bbx_2,...,\bbx_2,...,\bbx_{n-1},\bbx_n,...,\bbx_n\}\\
Y&=\{y_{1, 1}, ..., y_{1, m_1}, y_{2, 1}, ..., y_{2, m_2}, ..., y_{n, 1}, ..., y_{n, m_n}\}
%
\end{aligned}
\end{equation}
%
be data generated from model:
%
\begin{equation}
\begin{aligned}
%
y_{i, j} &= f(\bbx_i) + \eta_{i,j} \text{ s.t. } i=1, ..., n ; j=1, ..., m_i ; \\
\eta_{i,j} &\sim \mathcal{N}(0, \sigma_i^2)
%
\end{aligned}
\end{equation}
%
Let:
%
\begin{equation}
\begin{aligned}
%
\hat{X}&=\{\bbx_1, \bbx_2, ..., \bbx_n\}\\
\hat{Y}&=\{\frac{1}{m_1} \sum_{j=1}^{m_1} y_{1, j}, ..., \frac{1}{m_n} \sum_{j=1}^{m_n} y_{n, j}\}
%
\end{aligned}
\end{equation}
%
be a compressed version of the data  generated from $f(\bbx_1)$, ...., $f(\bbx_n)$ with noise $\hat\eta_{i} \sim \mathcal{N}(0, \frac{\sigma_i^2}{m_i})$.
Let $\bbf_*$ be vector of latent value over $X_*$, then $\bbf_* | X, Y$ and $\bbf_* | \hat{X}, \hat{Y}$ have the same distribution $\mathcal{N}(\bbmu, \bbSigma)$, i.e.:
%
\begin{equation}\label{mainmainEQ}
\begin{array}{l}
\bbmu = M(\hat{X_*}) +\\
K(X_*, \hat{X}) (\diag(\bbsigma) + K(\hat{X}, \hat{X}))^{-1}(\bbzeta - M(\hat{X}))\\
\text{, where }  \zeta_i := \frac{1}{m_i} \sum_{j=1}^{m_i} y_{i, j}, \bbsigma=[\frac{\sigma_1^2}{m_1}, ..., \frac{\sigma_n^2}{m_n}]^T\\
\bbSigma = K(X_*, X_*) -\\
K(X_*, \hat{X}) (\diag(\bbsigma) + K(\hat{X}, \hat{X}))^{-1} K(\hat{X}, X_*)
\end{array}
\end{equation}
%
\end{theorem}
%
%
\begin{proof}
We provide proof for $m(\bbx)=0$ case, general result could be concluded similarly.
%
\begin{equation}\label{logEq}
\begin{aligned}
%
\mathbb{P}(\bbf_*, \bbf, Y | X) = \mathbb{P}(Y|\bbf)&\mathbb{P}(\bbf_*, \bbf|X_*,X)\\
\log\mathbb{P}(\bbf_*, \bbf, Y | X)= \sum_{i=1}^n\sum_{j=1}^{m_i}& -\frac{1}{2}\frac{(y_{i,j}-f(\bbx_i))^2}{\sigma_i^2}\\
-\frac{1}{2} \begin{bmatrix} \bbf\\ \bbf_* \end{bmatrix}^T  \begin{bmatrix}\bbOmega_{11} & \bbOmega_{12} \\ \bbOmega_{12}^T & \bbOmega_{22}\end{bmatrix}&\begin{bmatrix} \bbf\\ \bbf_* \end{bmatrix}+Constant
%
\end{aligned}
\end{equation}
, where $\begin{bmatrix} K(X,X) & K(X, X_*)\\ K(X_*, X)&K(X_*, X_*) \end{bmatrix}^{-1}=\begin{bmatrix}\bbOmega_{11} & \bbOmega_{12} \\ \bbOmega_{12}^T & \bbOmega_{22}\end{bmatrix}$. Let $\bbH$ be $\sum_{i=1}^n m_i \times n$ matrix such that $\bbH_{(\sum_{k=0}^{i-1}m_k+j),i}=\frac{1}{\sigma_i^2}$ for $i=1, ..., n ; j=1, ..., m_i$ and rest of its entries are zero, additionally let $\bby=[y_{1,1},..., y_{n, m_n}]^T$. We can rewrite equation~\ref{logEq} as:
\begin{equation}\label{logEq}
\begin{aligned}
%
&\log\mathbb{P}(\bbf_*, \bbf, Y | X)=\\
%
& -\frac{1}{2} \begin{bmatrix}\bby\\ \bbf\\ \bbf_* \end{bmatrix}^T  \begin{bmatrix}\diag(\frac{1}{\sigma_1^2},...,\frac{1}{\sigma_n^2}) & -\bbH & \bb0 \\ -\bbH^T & \diag(\bbsigma)^{-1} & \bb0\\ \bb0 & \bb0 &\bb0 \end{bmatrix}\begin{bmatrix}\bby\\ \bbf\\ \bbf_* \end{bmatrix}\\
%
&-\frac{1}{2} \begin{bmatrix}\bby\\ \bbf\\ \bbf_* \end{bmatrix}^T  \begin{bmatrix}\bb0 & \bb0 & \bb0\\ \bb0 & \bbOmega_{11} & \bbOmega_{12} \\ \bb0 & \bbOmega_{12}^T & \bbOmega_{22}\end{bmatrix}\begin{bmatrix}\bby\\ \bbf\\ \bbf_* \end{bmatrix}+Constant\\
%
%
%
&= -\frac{1}{2} \begin{bmatrix}\bby\\ \bbf\\ \bbf_* \end{bmatrix}^T \hat \bbOmega \begin{bmatrix}\bby\\ \bbf\\ \bbf_* \end{bmatrix} + Constant \\
%
&\text{, where } \hat \bbOmega = \begin{bmatrix}\diag(\frac{1}{\sigma_1^2},...,\frac{1}{\sigma_n^2}) & -\bbH & \bb0 \\ -\bbH^T & \bbOmega_{11}+\diag(\bbsigma)^{-1} & \bbOmega_{12}\\ \bb0 & \bbOmega_{12}^T & \bbOmega_{22} \end{bmatrix}
\end{aligned}
\end{equation}
%
, which means $\begin{bmatrix}\bby\\ \bbf\\ \bbf_* \end{bmatrix} \sim \mathcal{N}(\bb0, \hat \bbOmega^{-1})$, so we can conclude that $\begin{bmatrix} \bbf\\ \bbf_* \end{bmatrix}| X, Y \sim \mathcal{N}(-\diag(\frac{1}{\sigma_1^2},...,\frac{1}{\sigma_n^2})^{-1}[\bbH,\bb0]\bby,  \begin{bmatrix}\bbOmega_{11}+\diag(\bbsigma)^{-1} & \bbOmega_{12}\\ \bbOmega_{12}^T & \bbOmega_{22} \end{bmatrix}^{-1})$. 
%
%
From definition $\bbH$ we can see that $\bbzeta=-\diag(\frac{1}{\sigma_1^2},...,\frac{1}{\sigma_n^2})^{-1}[\bbH,\bb0]\bby$, so we see $\begin{bmatrix} \bbf\\ \bbf_* \end{bmatrix}| X, Y \sim \mathcal{N}(\bbzeta,  \begin{bmatrix}\bbOmega_{11}+\diag(\bbsigma)^{-1} & \bbOmega_{12}\\ \bbOmega_{12}^T & \bbOmega_{22} \end{bmatrix}^{-1})$. 
%
%
If we follow the same path for second data set we can see that $\begin{bmatrix} \bbf\\ \bbf_* \end{bmatrix}| \hat{X}, \hat{Y} \sim \mathcal{N}(\bbzeta,  \begin{bmatrix}\bbOmega_{11}+\diag(\bbsigma)^{-1} & \bbOmega_{12}\\ \bbOmega_{12}^T & \bbOmega_{22} \end{bmatrix}^{-1})$. We see that  $\begin{bmatrix} \bbf\\ \bbf_* \end{bmatrix}| \hat{X}, \hat{Y}$ and $\begin{bmatrix} \bbf\\ \bbf_* \end{bmatrix}| X, Y$ have the same distribution, so by integrating out $\bbf$ in both distributions we can conclude $\bbf_* | X, Y$ and $\bbf_* | \hat{X}, \hat{Y}$ have the same distributions. In order to make sure about equation~\ref{mainmainEQ}, reader may do the integration part precisely. 
%
\end{proof}
%
%
%
%
%_______________________________________________________________________________________________________________
%
%______________________________________
\def\D{{\ensuremath{diag(\bfnu_{t,c})}}}
\def\V{{\ensuremath{\mathbf v}}}
\def\ind{{\ensuremath{\mathbf {Ind}}}}
%______________________________________
%
%
%
%
At time step $t$ let $\setP_{t,c}$ be set of pseudo points in $\cup_{l=0}^t\setD_{l,c}$ (without repetition), i.e. $\setP_{t,c}=\{\bbx|(\bbx,y)\in\cup_{l=0}^t\setD_{l,c}\}$, $\bbmu_{t,c}\in \reals^{|\setP_{t,c}|}$ be array of mean of measurements, and $\bbnu_{t,c}\in \reals^{|\setP_{t,c}|}$ be array of number of observations corresponding with pseudo points in $\setP_{t,c}$. Then we can do test prediction by replacing $\setP$,$\bbmu$,$\bbnu$ with $\setP_{t,c}$,$\bbmu_{t,c}$,$\bbnu_{t,c}$ respectively in \textit{Theorem}~\ref{main}.
%
%
%
%
Information gathering is to keep track of $\bbmu_{t,c}$,$\bbnu_{t,c}$. In order to do prediction for unseen points we need to keep track of matrix $\bbOmega_{t,c}=(\sigma^2\D^{-1}+K_{\setP_{t,c}\setP_{t,c}})^{-1}$ lets call it \textit{Extended Information Matrix}.
\textcolor{blue}{this is actually the precision matrix of the GP, right ? Why not call it Precision matrix?}
%
%
%
%
\subsection{Information gathering at time step $t$}
%
We keep the mean and number of observations for pseudo points in $\bbmu_c$ and $\bbnu_c$ respectively. \textcolor{blue}{How do $\bbmu_c$ and $\bbnu_c$ relate to the GP a posteriori updates in the preceding subsection? That is ambiguous here.} At every time step $t$, $\bbmu_c = \bbmu_{t,c}$, and  $\bbnu_c = \bbnu_{t,c}$. Before receiving new data $\setD_{t,c}$, we have $\bbmu_{t-1,c}$,$\bbnu_{t-1,c}$, and $\setP_{t-1,c}$. In new data we see some pseudo points for first time $\setP_{t,c}^{new}=\{\bbx|(\bbx,y)\in\setD_{t,c}\} \slash \setP_{t-1,c}$, for each of which, one zero element we will add to $\bbmu_c$,$\bbnu_c$. Then for each element of $\{\bbx|(\bbx,y)\in\setD_{t,c}\}$ with index $j$ in $\bbmu_c$,$\bbnu_c$ we will update $\bbmu_{t,c}=\frac{\bbmu_{c}\bbnu_{c}+y}{\bbnu_{c}+1}$, and $\bbnu_{t,c}=\bbnu_{c}+1$. \textcolor{blue}{some reference to the appropriate parametric update of a GP is missing here, so interpreting these applications of Bayes rule is a little unclear.}
%
%
%
%
\subsection{Extended Information Matrix Update}
%
Based on the time we want to compute the probabilistic semantic label of an unseen point, two situations may arise: 
%
%
\begin{enumerate}
%
\item Offline learning: we first collect data up to some time horizon, which forms the static prior for computing the posterior mean and covariance at an unseen point; 
%
\item Online learning: the prior dynamically evolves according to each new observation, i.e., training and testing are concurrent. 
%
\end{enumerate}
%
%
%
%
\textcolor{blue}{you need to recall the definition of $\bbOmega_c$ here. You define it in Corollary 1 but need to reiterate what it is and why it's important here.}
In first case we can calculate the $\bbOmega_c$ at the end, but in second case calculating $\bbOmega_c$ after each observation is very un efficient. In continue we will introduce the most efficient way to do this updating after each observation. We have two case that $\bbOmega_c$ changes, we either see another observation of existing pseudo point, or we see new pseudo points.
%
%
%
%
%________________________________________________________________________________________________
\subsubsection{Update an existing pseudo point}
%
Lets assume we have $r$ more observations of the $i$'th pseudo point. Based on definition of the Extended Information Matrix we want to calculate: 
%
\begin{equation}
\begin{aligned}\label{addoneObs}
%
    \bbOmega_c^{new}&=(\bbOmega_{t,c}^{-1}+\delta \bfe_i \bfe_i^\top)^{-1}\\
    %
    &= \bbOmega_{t,c}-\frac{1}{\frac{1}{\delta}+\bfe_i^\top\bbOmega_{t,c}\bfe_i}\bfe_i^\top\bbOmega_{t,c}\bbOmega_{t,c}\bfe_i
    %
\end{aligned}
\end{equation}
%
%
%
%
%
In especial case when the number of observations is one then $\delta =\frac{-\sigma^2}{\D[i](\D[i]+1)}$
%
%
%
%
%________________________________________________________________________________________________
%
%
%
%
\subsubsection{Adding a set of pseudo points}
%
We want to add a set of pseudo points $P'$ let $B=K_{\setP_{t,c}P'}$ and $C=\sigma^2\diag(\bbnu')^{-1} + K_{P'P'}$ where $\bbnu'$ is array of number of observation for pseudo points in $P'$. The new $\bbOmega_c$ will be:
%
%
%
%
\begin{equation}
\begin{aligned}\label{goodequation}
%
    \bbOmega_c^{new} &= \begin{bmatrix}
    %
    \bbOmega_{t,c}^{-1} & B \\
    %
    B^T & C
    %
  \end{bmatrix}^{-1}\\
  %
  &=\begin{bmatrix}
  %
    E& F \\
    %
    F^T& G
    %
  \end{bmatrix}\\
  %
  E&=\bbOmega_{t,c}+ \bbOmega_{t,c}B(C-B^T \bbOmega_{t,c}B)^{-1}B^T \bbOmega_{t,c}\\
  %
  F&=-\bbOmega_{t,c}B(C-B^T \bbOmega_{t,c}B)^{-1}\\
  %
  G&=(C-B^T \bbOmega_{t,c} B)^{-1}\\
  %
\end{aligned}
\end{equation}
%
%
%
\textcolor{blue}{remove the number of equation numbers in the preceding sequence to at most one. Also, you need to add a few comments about what the equations are or what they mean after they are presented. Otherwise, it is impossible to know what you're saying.}
%
%
And note that we can not do better since any way we need to calculate the inverse of new pseudo points which is $\ccalO(|P'|^3)$ and we need to provide the covariance matrix related to the relation from the old pseudo points and the new ones which is $\ccalO(|P||P'|)$
%
%
%
%.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  S  E  C  T  I  O  N%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Deleting a set of pseudo points}
%Lets assume we have the inverse of covariance matrix $A=\begin{bmatrix} A_{new}^{-1} & B \\ B^T & C \end{bmatrix}^{-1}=\begin{bmatrix} A_{11}& A_{12} \\ A_{12}^T & A_{22} \end{bmatrix}$ in which $C$ represents the columns and rows corresponding to the pseudo points we want to eliminate, so we have $A$ and we want $A_{new}$ which is the inverse of covariance matrix corresponding to pseudo points with regard to equation\ref{goodequation} we see $A_{new} = A_{11} - A_{12}A_{22}^{-1}A_{12}^T$
%which is $\ccalO(|P'||P|^2)$.

\label{sec:gpblock}



==> tex_multi/DistributedGP_old.tex <==
% !TeX spellcheck = <none>
%!TEX root = ../main.tex
\section{Distributed Incremental GP Regression}
\label{sec:DistributedGP}
%
In the sparse GP formulation with pseudo-points in~\eqref{eq:pseudopoint_gp_posterior}, the posterior is determined by parametric updates for the posterior mean and covariance whose empirical kernel map and kernel matrices are evaluated only at pseudo-inputs  in~\eqref{eq:pseudopoint_distribution}. 
%
%
In previous sections, when all data is acquired by a single robot $\rb$, specifically, this amounts to an update rule for a GP at time step $t$ given its previous inference $\mu^\rb_{t-1}(\bbx), k^\rb_{t-1}(\bbx, \bbx')$, and new observation $\X[\rb]{t}, \tilde{\bfy}_{t}^\rb$. 

On the other hand, when multiple robots acquire observations via their on-board sensors and share information with neighboring robots, then the  information at a single robot's disposal is the collection of neighbors' posterior parameters $\left\{\mu^\rbsec_{t-1,\cls}(\bfx), k^\rbsec_{t-1,\cls}(\bfx,\bfx') | \rbsec \in \mathcal{N}_\rb \right\}$ as well as its own local observation sequence.

In this section, we develop a distributed GP inference technique by exploiting the relationship between Bayesian belief propagation in multi-agent settings and weighted averaging-based parametric update rules for the local GP mean and covariance of restricted to pseudo-point subspaces. The main innovation is the update rule of one robot's GP in terms of the parameters of its neighbors' posteriors.
%

%
\subsection{Network Model and Belief Propagation}
Multi-agent belief propagation in the case of fixed-dimension parametric updatees for linear statistical models amounts to decentralized implementations of stochastic mirror descent which incorporate weighted averaging rules. First, we define key quantities for its development before shifting to explaining how these techniques come to bear on decentralized updates for GPs. 

Begin then by defining a weight matrix $\weight$ associated with the network, which we assume is strongly connected. That is, there is a directed path connecting any two arbitrary nodes s, t of the graph. To define the weight matrix, we first define as $A$ the adjacency matrix of the graph (note that $a_{\rb\rbsec}$ are not necessary integers) and  $D = \diag(d_1, ... , d_n)$ as the degree matrix of the graph i.e. $d_i = \sum_{\rbsec\neq \rb} a_{\rb\rbsec}$. Further define $L=D-A$ as the Laplacian of the graph, which satisfies the property that $L \mathbf{1} = \bb0$. Let $\Delta = \max(d_1, ... , d_n)$. Then define the weight matrix as $\weight = I - \nu L$ for $0 \leq \nu \leq \frac{1}{\Delta}$. Observe that $\weight$ is row stochastic nonnegative matrix and primitive (so it has a stationary distribution). These conditions arise in the analysis of distributed gradient descent algorithms as well as Perron-Frobenius theory. 

\begin{remark}\label{remark:network} (Static Versus Time-Varying Networks)In this paper, for simplicity, we restrict focus to the case that the weight matrix does not change over time. However, our method could be generalized to time variant graphs with specific conditions on changing weight matrices, by considering the stationary distribution of weight matrices at each time step instead of a single stationary distribution. This complication we defer to future work.
\end{remark}
%
%
%
\subsubsection{Fixed-Dimension Normal Update}
\label{NormalUpdate}
For the purpose of exposition, consider the case where robot $i$ seeks to track a fixed-dimensional hidden (random) vector $y$ via local observations $z_t^i$. To do so in a Bayesian manner under a linear observation model, we specify that the initial local likelihood $p^\rb_0$ on $y$ has a Normal prior, which gives rise to the linear measurement model:
\begin{equation}
\begin{aligned}
z^\rb_t = H^\rb  y_t+ v^\rb, \quad v^\rb \sim \mathcal{N}(0, V^\rb)
\end{aligned}
\end{equation}
as in  \cite{atanasov2014joint}. Then, we consider a Bayesian belief propagation setup in which each robot seeks to infer the distribution  of $y$ with respect to its neighbors through the geometric mean weighting rule: 
\begin{equation}\label{eq:belief_propagation}
\begin{aligned}
p^\rb_{t+1}(y) \varpropto \phi^\rb(z^\rb_{t+1}|y) \prod_{\rb=1}^n (p^\rb_t(y))^{\weight_{\rb\rbsec}}
\end{aligned}
\end{equation}
%
where $\phi^\rb( . |y)$ is the Normal density function evaluated at local observation $z^\rb_{t+1}$ . At each time step, this approach leads to linear update on information mean $\bfomega_{t+1}^\rb $ and information matrix $\Omega_{t+1}^\rb$ of normal distributions on the $y$. To be specific, by exploiting the relationship between the geometric means of the likelihood and the parametric updates for the means and covariances, we may write the following recursion:
%
%
\begin{equation}\label{eq:normalUpdate}
\begin{aligned}
\bfomega_{t+1}^\rb &= \sum_{\rb=1}^n\weight_{\rb\rbsec} \bfomega_{t}^\rbsec + {H^\rbsec}^\top {V^\rbsec}^{-1}z^\rbsec_t \\
\Omega_{t+1}^\rb &= \sum_{\rbsec=1}^n\weight_{\rb\rbsec} \Omega_{t}^\rbsec + {H^\rbsec}^\top {V^\rbsec}^{-1} {H^\rbsec}
\end{aligned}
\end{equation}

The preceding expression in \eqref{eq:normalUpdate} is shown to yield consistent estimates in the sense that each agent's local estimate attains mean square error comparable to a centralized offline one with all information aggregated in advance  \cite{atanasov2014joint}. Unfortunately, this update scheme cannot be directly applied to the GP setting due to the presence of non-fixed parameter dimension associated with concatenation of past observations inherent to GP parametric updates and the hierarchical octree pseudo-point approximations used to efficiently parameterize the GP in preceding sections.

%\subsection{Multi-Agent Belief Propagation}
%We can not use Atanasov et al.~\cite{atanasov2014joint}'s approach directly, since it assumes the dimension of phenomenon is fixed.
%This means each robot has to update over all the possible pseudo points $\allPs$ which is very inefficient. Because the effect of the most of the $\allPs$ is negligible. We are not aware of the effective pseudo points at the beginning, so we assume we will receive them over time. Employing GP helps us to address unfixed dimensional problem, we have.

%
%
%
%
\subsubsection{Gaussian Process Network Update}
In order to extend the introduced idea in Sec.~\ref{NormalUpdate} to become suitable for non-parametric method GP, we consider the implications of \eqref{eq:belief_propagation} to write updates for robot $i$ based on its local observations and weighted averaging of its posterior parameters restricted to the appropriate local pseudo-point subspace. To do so, note that in  \eqref{eq:pseudopoint_distribution} and \eqref{eq:pseudopoint_gp_posterior}, the posteriori is defined by the parameters $\Gamma$ and $\bbgamma$. Thus, by sequentially updating $\Gamma$ and $\bbgamma$ via local observations and incorporation of neighbors' distributional parameters $\Gamma$ and $\bbgamma$, then  \eqref{eq:pseudopoint_gp_posterior} becomes executable.

To be more specific, in the decentralized incremental setting under consideration, each robot $\rb$ receives local data $\tilde{\calX}_t^\rb$, $\tilde{\bfy}_t^\rb$ sequentially and maintains a Gaussian density $p_t^\rb(\bff_t^\rb) := p(\bff_t^\rb | \Theta_t^\rb)$ with parameters $\Theta_t^\rb := (\calP_t^\rb, \bfm_t^\rb, \bfzeta_t^\rb)$ over the latent function value $\bff_t^\rb := f(\calP_t^\rb)$  at the pseudo points $\calP_t^\rb$. For simplicity we assume $\mu_0(\bbx) = 0$. The parameters $\Theta_t^\rb$ are sufficient to specify the mean and covariance of $\bff_t^\rb$ via \eqref{eq:compressed_gp_posterior}:
\begin{equation}
\label{eq:meanForRobotsPs}
\begin{aligned}
\bfmu_t^\rb &= k_0(\calP_t^\rb,\calP_t^\rb)Z_t^\rb\bfzeta_t^\rb \\
\Sigma_t^\rb &=  k_0(\calP_t^\rb,\calP_t^\rb) - k_0(\calP_t^\rb,\calP_t^\rb)Z_t^\rb k_0(\calP_t^\rb,\calP_t^\rb)
\end{aligned}
\end{equation}
or equivalently:
\begin{equation}
\label{eq:gammaForRobots}
\begin{aligned}
\bfgamma_t^\rb &= k_0(\cP[\rb]{t},\cX[\rb]{t})\prl{\sigma^2I}^{-1}\bby^\rb_t\\
&= k_0(\cP[\rb]{t},\cP[\rb]{t})\prl{\sigma^{-2}\diag(\bfm_t^\rb)}\bfzeta^\rb_t\\
\Gamma_t^\rb &=  k_0(\cP[\rb]{t},\cX[\rb]{t})\prl{\sigma^2 I}^{-1}k_0(\cX[\rb]{t},\cP[\rb]{t})\\
&=  k_0(\cP[\rb]{t},\cP[\rb]{t})\prl{\sigma^{-2}\diag(\bfm_t^\rb)}k_0(\cP[\rb]{t},\cP[\rb]{t})
\end{aligned}
\end{equation}
If the training data is generated as in Sec.~\ref{sec:algorithm}, such that all observations come from locations in $\calP_t^\rb$, then $\Lambda_t^\rb = 0$ in \eqref{eq:pseudopoint_distribution}.

%or equivalently the pseudo point information mean and information matrix:
%\begin{equation}
%\begin{aligned}
%\bfomega_t^k &= k_0(\calP_t^k,\calP_t^k)^{-1}\mu_0(\calP_t^k) + \frac{1}{\sigma^2}\diag(\bfm_t^k)\bfzeta_t^k\\
%\Omega_t^k &= k_0(\calP_t^k,\calP_t^k)^{-1} + \frac{1}{\sigma^2}\diag(\bfm_t^k)
%\end{aligned}
%\end{equation}

%
%\subsection{Distributed Gaussian Inference}
%\subsection{Distributed Incremental GP Regression}


%\subsection{pre}

%\blue{The duality between normal distribution on pseudo points and GP on them:  In comparison between of the Eq.~\eqref{eq:pseudopoint_distribution} and Eq.~\eqref{eq:pseudopoint_gp_posterior} we see that all the inference in both of them are in the $\Gamma$ and $\bbgamma$ which forms a duality between them. The main idea in updating the Gaussian Process between neighbors is to find the equivalence updating rule of the geometric mean with regard for $\Gamma$ and $\bbgamma$ when we consider the normal distribution of the pseudo points. Since we have the updated $\Gamma$ and $\bbgamma$, and all the inference we need for GP is in them, we have the updated GP.}
%
%
%
%
%
%In order to update the normal distribution of robot $k$ on its pseudo points $p^k_{t}$ with respect to its neighbors' distributions, at first we should make them the same dimension. In this regard first we 
%, in \eqref{eq:gammaForRobots} we have explained how to update the inference of robot $k$ i.e. $\bbgamma_t^k, \Gamma_t^k$ with regard to its own observations
{\noindent \bf Update for Static Pseudo-inputs.}
Suppose for the moment that the set of pseudo-points $\hat\calP$ is fixed for all the robots. Then, to update the inference of robot $\rb$ with respect to its neighbors' inferences may be computed in terms of the posteriors $\hat\bbf$ of other robots formulated with own observed data, i.e. $p_t^\rbsec(\hat\bbf)$ with their $\Gamma^\rbsec_{t}, \bbgamma^\rbsec_{t}$ such that $1 \leq \rbsec \leq n, \rbsec \neq \rb$. To propagate the information from the distinct local models, we consider a local likelihood estimate $p^\rb_{t+1}$ with $\Gamma^\rb_{t+1}, \bbgamma^\rb_{t+1}$ that is comprised of the product over the marginals of other agents with each factor taken to the power associated with weight $\mathbf{W}_{ij}$, i.e., the geometric average:
%
\begin{equation}
\begin{aligned}
p^\rb_{t+1}(\hat\bbf) \varpropto \prod_{ \rbsec \in \mathcal{N}_\rb\cup\{\rb\}} (p_t^\rbsec(\hat\bbf))^{\weight_{\rb\rbsec}}
\end{aligned}
\end{equation}
%
%
where $\weight$ is the previously defined weight matrix of the network. %such that $\weight_{\rb\rbsec} \geq 0$, $\sum_{\rbsec \in \mathcal{N}_\rb\cup\{\rb\}} \weight_{\rb\rbsec}=1$ (row stochastic nonnegative matrix) and $\weight$ has a stationary distribution $\pi$, i.e., $(\weight^\infty)_{\rb,\rbsec}=\pi_\rbsec$. 
%
%Using $\varpropto$ is because $p^k_{t+1}(\hat\bbf)$ must be a valid pdf (with its integral to be $1$), so there might be a coefficient difference between two sides of $\varpropto$\NA{This sentence is too far away from (23). You can also just comment it out since this is obvious.}. 
Since the product of Normal distributions of is Normal, we may then write $p^\rb_{t+1}(\hat\bbf) = \phi(\hat\bbf | \bbmu^\rb_{t+1}, \bbSigma^\rb_{t+1})$ as a Normal as well, with parameters defined by:

\begin{equation}
\begin{aligned}
(\bbSigma^\rb_{t+1})^{-1} &= \sum_{ \rbsec \in \mathcal{N}_\rb\cup\{\rb\}}\weight_{\rb\rbsec} (\hat{K}( \hat{K}+\Gamma^\rbsec_t)^{-1} \hat{K})^{-1}\\
&= \hat{K}^{-1}( \hat{K}+\sum_{ \rbsec \in \mathcal{N}_\rb\cup\{\rb\}}\weight_{\rb\rbsec}\Gamma^\rb_t) \hat{K}^{-1}\\
%
(\bbSigma^k_{t+1})^{-1} \bbmu^\rb_{t+1} &= \sum_{ \rbsec \in \mathcal{N}_\rb\cup\{\rb\}}\weight_{\rb\rbsec} (\hat{K}( \hat{K}+\Gamma^\rbsec_t)^{-1} \hat{K})^{-1}\\ 
&\quad \hat{K}{(\hat{K}+\Gamma^\rbsec_t)}^{-1}\bbgamma^\rbsec_t \\
&= \hat{K}^{-1}  (\sum_{ \rbsec \in \mathcal{N}_\rb\cup\{\rb\}}\weight_{\rb\rbsec}\bbgamma^\rbsec_t)
\end{aligned}
\end{equation}
%
where $\hat{K} = k_0(\hat\calP,\hat\calP)$. This is the GP analogue of the weighted averaging update rule in the case of linear statistical models given in \eqref{eq:normalUpdate}. By comparing the recent result with \eqref{eq:meanForRobotsPs} and \eqref{eq:gammaForRobots} we see that this geometric averaging is equivalent to:
\begin{equation}
\begin{aligned}
\Gamma^\rb_{t+1} &= \sum_{ \rbsec \in \mathcal{N}_\rb\cup\{\rb\}}\weight_{\rb\rbsec}\Gamma^\rbsec_t \\
\bbgamma^\rb_{t+1} &= \sum_{ \rbsec \in \mathcal{N}_\rb\cup\{\rb\}}\weight_{\rb\rbsec}\bbgamma^\rbsec_t \;.
\end{aligned}
\end{equation}
%
%
After robot $\rb$ incorporates the information of its neighbors, then it increments its distributional parameters in accordance with new observation $\X[\rb]{t+1}, \tilde{\bfy}_{t+1}^\rb$. Suppose for now that the number of pseudo-points is fixed, i.e. $\P[\rb]{t}\subset \hat\calP$. Then,  \eqref{eq:gammaForRobots} implies that we add $k_0(\hat\calP, \X[\rb]{t+1})(\sigma^2I)^{-1} \tilde{\bfy}_{t+1}^\rb$ to $\bbgamma^\rb_{t+1}$ and $k_0(\hat\calP, \X[\rb]{t+1})(\sigma^2I)^{-1} k_0(\X[\rb]{t+1},\hat\calP)$ to $\Gamma^\rb_{t+1}$. Taken together, then, we have the decentralized incremental update for the GP representation of robot $\rb$ for its parameters $\bbgamma^\rb_t, \Gamma^\rb_t$ as: 

\begin{align}\label{eq:updateSensors}
\bbgamma^\rb_{t+1} &= \sum_{ \rbsec \in \mathcal{N}_\rb\cup\{\rb\}} \weight_{\rb\rbsec}\bbgamma^\rbsec_{t} + k_0(\hat\calP, \X[\rb]{t+1})(\sigma^2I)^{-1} \tilde{\bfy}_{t+1}^\rb\\
\Gamma^\rb_{t+1} &= \sum_{ \rbsec \in \mathcal{N}_\rb\cup\{\rb\}} \weight_{\rb\rbsec}\Gamma^\rbsec_{t} +  k_0(\hat\calP, \X[\rb]{t+1})(\sigma^2I)^{-1} k_0(\X[\rb]{t+1},\hat\calP)\notag
\end{align}

%
%
%
%
{\noindent \bf Update for Dynamic Pseudo-inputs.}
Up until now, we have restricted focus to the case where the set of pseudo-points is fixed when executing an update. Now we consider how these expressions must be augmented when the set of pseudo-points changes. To do so, we first note that by the definition $\bbgamma^\rb_{t}, \Gamma^\rb_{t}$, the structure of the updates is unchanged when the set of pseudo-points $\cP[\rb]{t}$ changes. That is, it is only a set function of $\cP[\rb]{t}$. Therefore, to increment pseudo-point set, we define the local aggregation of pseudo-points at robot $i$ as the set union  $\hat\calP = \cP[\rb]{t+1} = \bigcup\limits_{\rbsec \in \mathcal{N}_\rb\cup\{\rb\}} \cP[\rbsec]{t}\cup\P[\rb]{t+1}$. Then, one may rewrite the parametric updates of neighbor's GPs via $\hat\calP$. Specifically, denote as $\hat\bbgamma^\rbsec_{t}, \hat\Gamma^\rbsec_{t}$ the GP parameters of robot $j$ evaluated at pseudo-points $\hat\calP$. Then, the update expression for non-static pseudo-point sets takes the form
%
\begin{align}
\cP[\rb]{t+1} &= \bigcup\limits_{\rbsec \in \mathcal{N}_\rb\cup\{\rb\}} \cP[\rbsec]{t}\cup\P[\rb]{t+1} \notag\\
\bbgamma^\rb_{t+1} &= \sum_{ \rbsec \in \mathcal{N}_\rb\cup\{\rb\}} \weight_{\rb\rbsec} \hat\bbgamma^\rbsec_{t} + k_0(\hat\calP, \X[\rb]{t+1})(\sigma^2I)^{-1} \tilde{\bfy}_{t+1}^\rb \label{eq:updategamma}\\
\Gamma^\rb_{t+1} &= \sum_{ \rbsec \in \mathcal{N}_\rb\cup\{\rb\}} \weight_{\rb\rbsec} \hat\Gamma^\rbsec_{t} +  k_0(\hat\calP, \X[\rb]{t+1})(\sigma^2I)^{-1} k_0(\X[\rb]{t+1},\hat\calP) \notag
\end{align}
%
One may rewrite the preceding expression in terms of the number of observations $m^\rb_{t+1}(\bfp)$ and mean observation $\zeta^\rb_{t+1}(\bfp) $ akin to \eqref{eq:update} via \eqref{eq:gammaForRobots} for the dynamic pseudo-point case as:
%
\begin{align}\label{eq:updaterule}
%\cP[\rb]{t+1} &= \bigcup\limits_{\rbsec \in \mathcal{N}_\rb\cup\{\rb\}} \cP[\rbsec]{t}\cup\P[\rb]{t+1}\notag\\ 
m^\rb_{t+1}(\bfp) &= \sum_{ \rbsec \in \mathcal{N}_\rb\cup\{\rb\}} \weight_{\rb\rbsec} m^\rbsec_t(\bfp) + \tilde{m}^\rb_{t+1}(\bfp)\\
\zeta^\rb_{t+1}(\bfp) &= \frac{\sum_{ \rbsec \in \mathcal{N}_\rb\cup\{\rb\}} \weight_{\rb\rbsec} m^\rbsec_t(\bfp)\zeta^\rbsec_t(\bfp) + \tilde{m}^\rb_{t+1}(\bfp)\tilde{\zeta}^\rb_{t+1}(\bfp)}{m_{t+1}^\rb(\bfp)}\notag
\end{align}
%
%
%``centralized estimation'' estimation
%
%
%
\subsubsection{Convergence to Centralized Estimation }
To evaluate the estimation accuracy of the proposed distributed sparse GP regression, we compare it versus centralized GP regression. At first we are going to define the centralized estimator, then we provide theoretical evidence of convergence of individual robots' estimation to the centralized estimation. Consider a centralized estimator that receives all robot observations at each time step and uses them to update a sparse GP distribution according to \eqref{eq:update}. This centralized estimator should have all the information in the network, so at each time step its observation should include all the observations that all the real robots in the network have. This centralized estimator also should be affected by $\weight$ matrix. If $\weight = \frac{1}{n}\boldsymbol{11^\top}$, it means the credibility of all robots are the same, which means observation of centralized estimator should be exactly the collection of all the robots' observations in the network. If $\weight$ is not uniform it means the credibility of all robots are not the same. In order to affect the credibility of robots we assume that the centralized estimator will consider the data from different robots with different noise variance. More precisely, variance noise from different robots are different proportional to $\pi$, the stationary distribution of the Perron matrix $\weight$. Observation of robot $\rb$ at time step $t$ is $\X[\rb]{t,\rbsec}, \Y[\rb]{t,\rbsec}, \P[\rb]{t,\rbsec}$. For tge mentioned observation, the difference for centralized estimator and the robot $\rb$ is in their noise variance. Centralized estimation observes this observation with noise variance $\frac{\sigma^2}{\pi_\rb}$ while the noise variance is $\sigma^2$ for the robot $\rb$. For notation simplicity, we assume all the observations have variance $\sigma^2$, but the number of centralized estimation could be non-integers, so for centralized estimation by $m^{ctr}_t(\bbp)$ we mean $\sigma^2$ divided by equivalent variance noise for point $\bbp$ at time $t$. For observation at time step $t$, this is equivalent to assume that the variance noise is $\sigma^2$ for centralized estimation, but the number of observation is $\pi_\rb\tilde{m}_\rb^t(\bbp)$, this way we can also define $\zeta^{ctr}_{t}(\bfp)$ based on \eqref{eq:update}:
%
%
\begin{equation}
	\label{eq:central}
	\begin{aligned}
		\cm[ctr]{t+1}(\bbp) &= \cm[ctr]{t}(\bbp)+\sum_{\rb=0}^n \pi_\rb\m[\rb]{t}(\bbp)\\
		\czet[ctr]{t+1}(\bbp) &= \frac{\cm[ctr]{t}(\bbp)\czet[ctr]{t}(\bbp)+\sum_{\rb=0}^n \pi_\rb\m[\rb]{t}(\bbp)\zet[\rb]{t}(\bbp)}{\cm[ctr]{t+1}(\bbp)}\\
	\end{aligned}
\end{equation}
%
%
%--------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%
First, we prove that the GPs of all robots, using the distributed updates in \eqref{eq:updaterule}, converge to centralized GP estimate as $t\to \infty$.
%
\begin{proposition}
\label{th:Net1}
If the network is updated through ~\eqref{eq:updaterule} and data streaming stops at some time $T < \infty$, then as $t\to \infty$ the Gaussian Process of each robot converges to the centralized estimation i.e. $\|\bfm_t^k - \bfm^{ctr}_t\| \to 0$ and $\|\bfzeta_t^k - \bfzeta^{ctr}_t\| \to 0$.
\end{proposition}
%
%
%
\begin{proof}
We just need to prove that $m^k_t(\bbp), \zeta^k_{t}(\bbp)$ converges to $m^{ctr}_t(\bbp), \zeta^{ctr}_{t}(\bbp)$ for any $\bbp\in\allPs$. 
Because, for a specific pseudo point $\bbp$, $m_t(\bbp)$ is never negative, and if $\bbp\in\cP{t}$ it is positive, additionally if $m_t(\bbp)$ is positive then $\bbp\in\cP{t}$. 
For a specific pseudo point $\bbp\in\allPs$ let write $\cm[ctr]{t}(\bbp), \zeta^{ctr}_{t}(\bbp)$ in terms of $\m[\rb]{t}(\bbp), \zet[\rb]{t}(\bbp)$. In this regard note that at each time step centralized estimation at each time step $t$ receives $\zet[\rb]{t}$ for all $\rb$, each with equivalent (when we assume the variance noise is $\sigma^2$ for the observation of the centralized estimation) number of observation $\pi_\rb \m[\rb]{t}$, so based on \eqref{eq:central} we have:
%
%
\begin{equation}
\label{eq:central-expansion}
\begin{aligned}
\cm[ctr]{t}(\bbp) &= \sum_{\tau=0}^{t}\sum_{\rb=0}^n \pi_\rb\m[\rb]{\tau}(\bbp)\\
\czet[ctr]{t}(\bbp) &= \frac{1}{\cm[ctr]{t}(\bbp)}\sum_{\tau=0}^{t}\sum_{\rb=0}^n \pi_\rb\m[\rb]{\tau}(\bbp)\zet[\rb]{\tau}(\bbp)\\
\end{aligned}
\end{equation}
%
%
Then, we write $\cm[\rb]{t}(\bbp), \czet[\rb]{t}(\bbp)$ in terms of $\m[\rb]{t}(\bbp), \zet[\rb]{t}(\bbp)$. In this regard note that the coefficient of $\m[\rbsec]{\tau}(\bbp)$ in $\cm[\rb]{t}(\bbp)$ with regard to update rule \eqref{eq:updaterule} is $(\weight^{t-\tau})_{\rb\rbsec}$ since it can propagate through the network with weight matrix $\weight$ and reach to robot $\rb$ via all paths with length $t-\tau$, so we have:
%
\begin{equation}
\label{eq:echo-k-expansion}
\begin{aligned}
\cm[\rb]{t}(\bbp) &= \sum_{\tau=0}^{t}\sum_{\rb=0}^n (\weight^{t-\tau})_{\rb\rbsec}\m[\rbsec]{\tau}(\bbp)\\
\czet[\rb]{t}(\bbp) &= \frac{1}{\cm[\rb]{t}(\bbp)}\sum_{\tau=0}^{t}\sum_{\rbsec=0}^n (\weight^{t-\tau})_{\rb\rbsec}\m[\rbsec]{\tau}(\bbp)\zet[\rbsec]{\tau}(\bbp)\\
\end{aligned}
\end{equation}
Since data collection will be stoped at some time $T$ (so, all $\X[\rb]{\tau}, \P[\rb]{\tau}$ are empty for all $\tau>T$), the convergence is concluded from the fact that $(\weight^{\infty})_{\rb\rbsec} = \pi_\rbsec > 0$. 
\end{proof}
%
%

\subsection{Fast Echoless Geometric Mean Update in GP Network}
%
In the previous section we explained how all robots should be updated in the multi-robot case. However, this is not efficient practically due to two reasons. Firstly, in order to all robots converge to central GP we should let the network updating goes on forever. Secondly, every time two robots communicate, they should pass all information that they have. It seems unnecessary, specifically we saw in proof of Prop.~\ref{th:Net1} that one observation is received infinite times (echos in the network).
%

In this regard we define a mini-batch of observation $\pck[\rb]{t}=\{\P[\rb]{t}, \m[\rb]{t}, \zet[\rb]{t}, list^\rb_t\}$ for each robot $\rb$. At time step $t$, it contains the robot's observation and list of robots that have already received this mini-batch. The $list^\rb_t$ is initialized by $\{\rb\}$. Additionally, for each robot $\rb$ we define a list of mini-batchs $\newpkg[\rb]{t}$ that contains the new mini-batchs that the robot should update its estimation with regard to them, and its previous version contains the old mini-batchs that the robot should transmit them to other robots.
%

Inspired by similarity of two \eqref{eq:central-expansion} and \eqref{eq:echo-k-expansion}, we manage that each mini-batch visits each robot in the network once (that is use of $list_t^\rb$ in $\pck[\rb]{t}$) rather than echoing in the network, and we pick the limit of $(\weight^{t-\tau})_{\rb\rbsec}$ in \eqref{eq:echo-k-expansion} as coefficient, so the convergence happens in finite and minimum time steps. The update for robot $\rb$ at time step $t$ is:
%
\begin{equation}
\label{eq:final_update_rule}
\begin{aligned}
\newpkg[\rb]{t+1} &= \bigcup\limits_{\pck[\rbsec]{\tau}\in\newpkg[r]{t}, r\in \mathcal{N}_\rb, \rb \notin list_\tau^\rbsec}\pck[\rbsec]{\tau} \cup \pck[\rb]{t+1}\\
list_\tau^\rbsec &= list_\tau^\rbsec \cup \{\rb\} \text{    for all } \pck[\rbsec]{\tau}\in \newpkg[\rb]{t+1}\\
\cP[\rb]{t+1} &= \bigcup\limits_{\pck[\rbsec]{\tau}\in \newpkg[\rb]{t+1}} \P[\rbsec]{\tau}\cup\cP[\rb]{t}\\
\cm[\rb]{t+1}(\bfp) &= m^\rb_{t}(\bfp) + \sum_{\pck[\rbsec]{\tau}\in \newpkg[\rb]{t+1}} \pi_{\rbsec} \tilde{m}^\rbsec_\tau(\bfp)\\
\czet[\rb]{t+1}(\bfp) &= \frac{\cm[\rb]{t}(\bfp) \czet[\rb]{t}(\bfp) + \sum\limits_{\pck[\rbsec]{\tau} \in \newpkg[\rb]{t+1}} \pi_{\rbsec} \m[\rbsec]{\tau}(\bfp) \zet[\rbsec]{\tau}(\bfp)}{\cm[\rb]{t+1}(\bfp)}
\end{aligned}
\end{equation}
%
%
%

\begin{corollary}
\label{cor:cnvrgn}
 If the network is updated through \eqref{eq:final_update_rule} such that data collection stops at time $t = T$, then at time $t = T+n-1$, the estimation of each robot converges to the centralized estimation i.e. $\|\bfm_t^k - \bfm^{ctr}_t\| \to 0$ and $\|\bfzeta_t^k - \bfzeta^{ctr}_t\| \to 0$.
\end{corollary}

\begin{proof}
let write $\cm[\rb]{t}(\bbp), \czet[\rb]{t}(\bbp)$ in terms of $\m[\rbsec]{\tau}(\bbp), \zet[\rbsec]{\tau}(\bbp)$. In this regard note that the important issue is to realize that whether the mini-batch $\pck[\rbsec]{\tau}$ is received by robot $\rb$ or not. Since the transition of mini-batchs are happening via matrix weight $\weight$, if corresponding element in $\weight^{t-\tau}$ i.e. $(\weight^{t-\tau})_{\rb\rbsec}$ is positive then the mini-batch received by the robot, otherwise (if it is zero) then it is not received. Let $\sign(x) = \begin{cases} 1 \text{ if } x>0 \\ 0 \text{ if } x=0\end{cases}$. For expansion of $\cm[\rb]{t}(\bbp), \czet[\rb]{t}(\bbp)$ when updated via \eqref{eq:final_update_rule} we can write:

%
%
\begin{equation}
\label{eq:k-expansion}
\begin{aligned}
\cm[\rb]{t}(\bbp) &= \sum_{\tau=0}^{t}\sum_{\rb=0}^n \sign((\weight^{t-\tau})_{\rb\rbsec}) \pi_\rbsec \m[\rbsec]{\tau}(\bbp)\\
\czet[\rb]{t}(\bbp) &= \frac{1}{\cm[\rb]{t}(\bbp)}\sum_{\tau=0}^{t}\sum_{\rbsec=0}^n \sign((\weight^{t-\tau})_{\rb\rbsec})  \pi_\rbsec \m[\rbsec]{\tau}(\bbp)\zet[\rbsec]{\tau}(\bbp)\\
\end{aligned}
\end{equation}
We assume $\weight^0=I$. Since data collection will be stoped at some time $T$ (so, all $\X[\rb]{t}, \P[\rb]{t}$ are empty for all $t>T$), in comparison with \eqref{eq:central-expansion} and \eqref{eq:k-expansion} the convergence is concluded from the fact that $(\weight^{n-1})_{\rb\rbsec} > 0$ (because the network is connected). 
%
%
\end{proof}






















==> tex_multi/NetworkUpdate.tex <==
%!TEX root = ../main.tex
\section{Network Update}
\label{sec:networkBackground}
%\NA{Why is this part of the background? No existing paper has ever discussed the multi-agent sparse GP inference. This is a major contribution of this work and should be presented as such. I recommend talking about adding and removing pseudo-points to the sparse GP inference approach before presenting the multi-agent setting. Similar to how you had adding and removing points around eq. (10). We should bring that information back.}
In the case that we have a network of sensors, through which they can communicate and share their information we have following method of updating the GP of each agent itself. In usual cases it is not efficient to update over all the possible $\calX_\#$, because effect of the most of the $\calX_\#$ is negligible. We are not aware of the effective pseudo points at the beginning, so we assume we will receive them over time.
%  

Let $\calX^k_{t,i}$ be set of pseudo points of agent $k$ until time $t$. To update $\bbgamma^k_{t,i}$ and $\Gamma^k_{t,i}$ with regard to the neighbors, first we extend $\calX^k_{t,i}$ such that it includes all the new pseudo points and pseudo points that the neighbors have as well, i.e.:
%
\begin{equation}
\begin{aligned}
%
\calX^k_{t+1,i} = \bigcup\limits_{j \in \mathcal{N}_k\cup\{k\}} \calX^j_{t,i}\cup\tilde\calX^k_{t,i}
%
\end{aligned}
\end{equation}
%
Then we update all $\bbgamma^j_{t,i}, \Gamma^j_{t,i}$ according to pseudo points $\calX^k_{t+1,i}$ to be $\hat\bbgamma^j_{t,i}, \hat\Gamma^j_{t,i}$ for $j \in \mathcal{N}_k\cup\{k\}$. In more details, based on~\eqref{eq:gamma} previously we had:
%
\begin{equation}
\begin{aligned}
%
\bbgamma^j_{t,i} &:= k(\calX^j_{t,i}, X^j_{t,i})(\Lambda^j_{t,i}+\sigma^2I)^{-1}\bby^j_{t,i}\\
%
\Gamma^j_{t,i} &:= k(\calX^j_{t,i}, X^j_{t,i})(\Lambda^j_{t,i}+\sigma^2I)^{-1}k(X^j_{t,i}, \calX^j_{t,i})
%
\end{aligned}
\end{equation}
%

By updating we mean:

%
\begin{equation}
\begin{aligned}
%
\hat\bbgamma^j_{t,i} &:= k(\calX^k_{t+1,i}, X^j_{t,i})(\Lambda^j_{t,i}+\sigma^2I)^{-1}\bby^j_{t,i}\\
%
\hat\Gamma^j_{t,i} &:= k(\calX^k_{t+1,i}, X^j_{t,i})(\Lambda^j_{t,i}+\sigma^2I)^{-1}k(X^j_{t,i}, \calX^k_{t+1,i})
%
\end{aligned}
\end{equation}
%

Now that we have everything with the appropriate dimension, we update the GP of agent $k$ with respect to its new observation and its neighbors in the network through:

\begin{equation}
\label{eq:updateSensors}
\begin{aligned}
\bbgamma^k_{t+1,i} &= \sum_{j \in \mathcal{N}_k\cup\{k\}} \kappa_{kj}\hat\bbgamma^j_{t,i}\\ 
&+ k(\calX^k_{t+1,i}, \tilde{X}^k_{t,i})(\Lambda^k_{t,i}+\sigma^2I)^{-1} \bby^{new}_{t,i}\\
\Gamma^k_{t+1,i} &= \sum_{j \in \mathcal{N}_k\cup\{k\}} \kappa_{kj}\hat\Gamma^j_{t,i} \\
&+  k(\calX^k_{t+1,i}, \tilde{X}^k_{t,i})(\Lambda^k_{t,i}+\sigma^2I)^{-1} k(\tilde{X}^k_{t,i},\calX^k_{t+1,i})
\end{aligned}
\end{equation}
where $\Lambda^k_{t,i} = \diag(\lambda(\tilde{X}^k_{t,i}))$ (when pseudo points are $\calX^k_{t+1,i}$).

%\subsection{Data Interpretation}
%With regard to Eq.~\ref{eq:gamma} and Eq.~\ref{eq:mu} we can uniquely describe the distribution with pseudo points $\calX_\#$ and data set $X,Y$ and their noise $\Phi$.
%Then Eq.~\ref{eq:updateSensors} is equivalent to:

%\begin{equation}
%\label{eq:equivalentUpdate}
%\begin{aligned}
%\calX_{t+1,i} &= \bigcup\limits_{j \in \mathcal{N}_i\cup\{i\}} \calX_{t,j}\bigcup\calX^{new}_{t,i}\\
%X_{t+1,i} &= \biguplus\limits_{j \in \mathcal{N}_i\cup\{i\}} X_{t,j} \biguplus X^{new}_{t,i}\\
%Y_{t+1,i} &= \biguplus\limits_{j \in \mathcal{N}_i\cup\{i\}} Y_{t,j} \biguplus Y^{new}_{t,i}\\
%\Phi_{t+1,i} &= \biguplus\limits_{j \in \mathcal{N}_i\cup\{i\}} \kappa_{ij}\Phi_{t,j} \biguplus \Phi^{new}_{t,i}\\
%\end{aligned}
%\end{equation}
%where $\Phi^{new}_{t,i} = \{\frac{1}{\lambda(\bbx)+\sigma^2}\}_{\bbx \in X^{new}_{t,i}}$.
%Which is equivalent to say:

%\begin{equation}
%\label{eq:equivalentUpdateCal}
%\begin{aligned}
%\calX_{t,i} &= \bigcup\limits_{l=0}^t\bigcup\limits_{j=1}^n\sign((\kappa^{t-l})_{ij})\calX^{new}_{l,j}\\
%X_{t,i} &=  \biguplus\limits_{l=0}^t\biguplus\limits_{j=1}^n\sign((\kappa^{t-l})_{ij})X^{new}_{l,j}\\
%Y_{t,i} &=  \biguplus\limits_{l=0}^t\biguplus\limits_{j=1}^n\sign((\kappa^{t-l})_{ij})Y^{new}_{l,j}\\
%\Phi_{t,i} &= \biguplus\limits_{l=0}^t\biguplus\limits_{j=1}^n (\kappa^{t-l})_{ij}\Phi^{new}_{l,j} 
%\end{aligned}
%\end{equation}

